Automating Dataset Updates Towards Reliable and Timely Evaluation of Large Language Models

Large language models (LLMs) have achieved impressive performance across various natural language benchmarks, prompting a continual need to curate more difficult datasets for larger LLMs, which is costly and time-consuming. In this paper, we propose to automate dataset updating and provide systematic analysis regarding its effectiveness in dealing with benchmark leakage issue, difficulty control, and stability. Thus, once the current benchmark has been mastered or leaked, we can update it for timely and reliable evaluation. There are two updating strategies: 1) mimicking strategy to generate similar samples based on original data, preserving stylistic and contextual essence, and 2) extending strategy that further expands existing samples at varying cognitive levels by adapting Bloom's taxonomy of educational objectives. Extensive experiments on updated MMLU and BIG-Bench demonstrate the stability of the proposed strategies and find that the mimicking strategy can effectively alleviate issues of overestimation from benchmark leakage. In cases where the efficient mimicking strategy fails, our extending strategy still shows promising results. Additionally, by controlling the difficulty, we can better discern the models' performance and enable fine-grained analysis neither too difficult nor too easy an exam can fairly judge students' learning status. To the best of our knowledge, we are the first to automate updating benchmarks for reliable and timely evaluation. Our demo leaderboard can be found at https://yingjiahao14.github.io/Automating-DatasetUpdates/.

==> chapters/dataset_bak.tex <==
% \section{Auto-question Generation Framework}
\section{Auto-Dataset Update Framework}
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.35]{figures/main_5.pdf}
    \caption{The auto-dataset update framework. For the mimicking strategy, we mimic the \uniformbox{F0F3BD}{0.2cm}{original test case} to get a similar but \uniformbox{58C09C}{0.2cm}{new sample}. For the Extending strategy, we extend the original sample to 
    multi-cognition levels (\uniformbox{FDF8E1}{0.2cm}{Remember \& Understand
    }, \uniformbox{FAEFBB}{0.2cm}{Apply}, \uniformbox{F6E694}{0.2cm}{Analysis}, \uniformbox{F4DD71}{0.2cm}{Evaluation}) to have a thorough and nuanced assessment.}
    \label{fig:framework}
\vspace{-5mm}
\end{figure*}

  In Figure~\ref{fig:framework}, there are two dataset update strategies: mimicking and extending. Both strategies are to generate new samples based on existing ones to mitigate overestimation when benchmark leakage happens. 
The mimicking strategy generates a similar yet unseen sample for each given sample, whereas the extending strategy aims at further controlling the cognitive levels of the sample generation.
Compared with mimicking strategy, extending strategy is beyond the scope of the given sample, challenging the model's capabilities in more nuanced and complex scenarios. We introduce these two strategies in Section~\ref{Mimic setting} and Section~\ref{Extend setting}, respectively. Then, we apply them to widely used benchmarks and manually analyze the quality (Section~\ref{sec: Updated Dataset Analysis}). Finally, we conduct experiments to verify their effectiveness, stability, and ability to deal with overestimation when benchmark leakage occurs (Section~\ref{section experiment}).

\subsection{Mimicking Strategy} \label{Mimic setting}
The mimicking strategy initiates by iterating through each sample in the selected dataset as a seed. This seed, combined with the corresponding task description (if have), forms the input for prompting LLMs~\cite{chatgpt} to generate new samples. Below is an example (more examples are shown in Appendix~\ref{sec case study}):
\begin{tcolorbox}[width=0.99\textwidth]
\textit{You are a question-writer expert. 
Please mimic the provided examples to generate *one* different but high-quality sample following the task description.} \\
\textit{\textbf{[Task Description]:}}
\textit{This task evaluates the model's ability to discern the plausibility of specific athletic actions based on the athlete's known skills and typical behaviors in their sport.  For example, a language model should understand that Leo Messi (arguably the best soccer player) is more likely to score goals or that basketball player Isaiah Thomas is unlikely to dunk (being a 5'9" point guard).}\\ 
\textit{\textbf{[Seed Sample]:}}
\textit{\{
        "input": "Jamal Murray was perfect from the line",
        "target\_scores": \{
            "plausible": 1,
            "implausible": 0
        \}
    \}}
 \\
\textit{\textbf{[New Generated Sample]:}}
\textit{\{"input": "Jamal Murray made 10 three-pointers in a row",
        "target\_scores": \{
            "plausible": 1,
            "implausible": 0
        \}
    \}}
\end{tcolorbox}

This strategy is designed to retain the stylistics and knowledge essential in the original ones, thus ensuring the quality of the new samples. After generation, we deploy validation strategies (details in Appendix~\ref{Mimic dataset}) to filter out answer-incorrect and duplicate samples.

\vspace{-2mm}
\subsection{Extending Strategy}\label{Extend setting}
Considering the limited data annotation ability, we adapt Bloom's taxonomy into LLMs evaluation with four cognitive levels. Figure~\ref{fig:framework} shows them with examples: \textbf{Remember and Understand Level} asks the model to list, recall basic concepts, interpret, summarize, and exemplify ideas or concepts; \textbf{Apply Level} tests the use of learned facts and abstractions in new contexts and particular situations; \textbf{Analysis Level} requires the model to break down concepts and examine the relationships among them; \textbf{Evaluation Level} asks the model to appraise a situation and criticize opinions or statements. Here to notice, Bloom's taxonomy is a theory that categorizes educational objectives into six levels of complexity and specificity: Remember, Understand, Apply, Analyze, Evaluate, and Create. For our purposes, we've combined the Remember and Understand levels for simplicity and excluded the Create level to more clearly distinguish between the different cognitive abilities we’re testing.
\begin{tcolorbox}[width=0.99\textwidth]
\textit{You are a question writer expert, your objective is to write **only one** really complex and difficult question about the given entity.  \\}
\textit{\textbf{[Generate Criterion]:} 
1. The question should be focused on the remember and understand level. This means the question should prompt for recall of facts, terms, and basic concepts, and NOT delve into deeper levels like Applying  Analyzing or Understanding. 
2. Ensure that you can confidently answer the questions you are proposing, if you can not answer it correctly or have no related knowledge about the entity please return "None". } \\
\textit{\textbf{[Seed Entity]:} Jamal Murray} \\
\textit{   
\textbf{[New Generated Sample]:} \{"question": What is the exact date, team and college that Murray was drafted into the NBA?, "ref\_answer": Answer... \}
}
\end{tcolorbox}
Given that each question in the original dataset is typically aligned with a specific cognitive level, this aspect presents a challenge for extending. 
To generate multi-level samples effectively, our approach involves abstracting the original question into a core entity, statement, or piece of knowledge. This abstraction can be done either manually or programmatically. Using this abstracted result, which serves as the seed, we guide LLMs to generate new questions focusing on different cognitive levels. Above is an example where we extract sports star ``Jamal Murray'' 
% (core entity) 
and prompt LLMs to extend (more examples are shown in Appendix~\ref{sec case study} and the detailed prompt is shown in Appendix~\ref{prompt appendix}).


It is important to note that our two strategies are efficient and adaptable, making them easily applicable across a wide range of benchmarks. 

\subsection{Apply to Existing Benchmarks}
To conduct auto-dataset update, we select BIG-Bench ~\cite{srivastava2023beyond} and MMLU~\cite{hendryckstest2021} as our seed datasets. From these benchmarks, we chose ten sub-tasks that are particularly representative of the diverse abilities LLMs are expected to demonstrate, ensuring a comprehensive evaluation. These tasks cover various types of questions, including both context-free and context-based, and assess the model's abilities in logical reasoning, common sense reasoning, memorization, mathematical ability, and more. A detailed analysis of the tasks is provided in Appendix~\ref{Mimic dataset}. Specifically, from BIG-Bench, we include:

\textbf{\href{https://github.com/google/BIG-bench/tree/main/bigbench/benchmark_tasks/sports_understanding}{Sports Understanding (Sports)}:} focuses on the ability to discern between plausible and implausible statements about sports stars.
\textbf{\href{https://github.com/google/BIG-bench/blob/main/bigbench/benchmark_tasks/periodic_elements/subtask_1/task.json}{Periodic Elements (Element)}:} measures knowledge of chemistry.
\textbf{\href{https://github.com/google/BIG-bench/tree/main/bigbench/benchmark_tasks/cs_algorithms/lcs}{CS Algorithms (Algos)}:} assesses models' understanding and utilization of computer science algorithmic concepts.
\textbf{\href{https://github.com/google/BIG-bench/tree/main/bigbench/benchmark_tasks/physical_intuition}{Physical Intuition (Phys)}:} tests the understanding of the physical behaviors.
\textbf{\href{https://github.com/google/BIG-bench/tree/main/bigbench/benchmark_tasks/elementary_math_qa}{Math Word Problems with Hints (Math)}:} tests the ability of models to perform mathematical reasoning in the context of arithmetic word problems. From the MMLU, we select five subtasks:
\textbf{Abstract Algebra (Algebra):} assesses models' understanding of abstract algebra concepts.
\textbf{International Law (Law):} evaluates models' ability to understand and follow rules and regulations.
\textbf{Econometrics (Econ):} tests the understanding of econometric principles and implications of econometric phenomena. 
\textbf{College Medicine (Medicine):} evaluates models' knowledge relevant to medicine.
\textbf{Computer Security (Security):} involves understanding the principles used to protect computer systems and networks.
After selecting datasets, we applied our two strategies to update these datasets and analyze the effectiveness and reliability of the updated samples.
\subsection{Updated Dataset Analysis}\label{sec: Updated Dataset Analysis}
% On one hand, 
We utilized ChatGPT (gpt-3.5-turbo) to apply the mimicking strategy for updating selected datasets from BIG-bench and MMLU. It's important to note that following the update process, we conducted a filtering step to remove duplicate and answer-incorrect samples, as detailed in Appendix~\ref{Mimic dataset}. This filtering process resulted in a dataset size smaller than the original. To achieve a dataset size comparable to the original, we literalize the dataset 2-3 times. (considering the time and the cost we limit the amount of the sample from the dataset ``Math'' to 1000). The statistical details of the updated datasets is shown in Table~\ref{table: mimic data}.

% \begin{table}[htb]
% \centering
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{lrr|lrr}
% \toprule
% \textbf{Task$_{\text{BIG}}$} & \textbf{\#Orig.} &\textbf{\#Mimic} & \textbf{Task$_{\text{MMLU}}$} & \textbf{\#Orig.} &\textbf{\#Mimic}\\
% \midrule
% Sports & 1000 & 951 & Algebra & 100 & 93\\
% Element &536  & 548 & Law & 121 & 117\\
% Algos & 320 & 300 & Econ & 114 & 101\\
% % conflict & 17528 & 1000 \\
% Phys & 81 & 99 & Medicine & 172 & 160\\
% Math & 7688 & 1016 & Security & 100& 100\\
% \bottomrule
% \end{tabular}}
% \caption{The statistical result of the original (Orig.)and mimicked (Mimic) ten subtasks from BIG-Bench and MMLU. For time and cost consideration, we limited the number of the generated samples on Math.}
% \label{table: mimic data}
% \end{table}
\begin{figure}[htb]
\vspace{-2mm}
\begin{minipage}[htb]{0.57\textwidth}
\small
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrr|lrr}
\toprule
\textbf{Task$_{\text{BIG}}$} & \textbf{\#Orig.} &\textbf{\#Mimic} & \textbf{Task$_{\text{MMLU}}$} & \textbf{\#Orig.} &\textbf{\#Mimic}\\
\midrule
Sports & 1000 & 951 & Algebra & 100 & 93\\
Element &536  & 548 & Law & 121 & 117\\
Algos & 160 & 150 & Econ & 114 & 101\\
% conflict & 17528 & 1000 \\
Phys & 81 & 81 & Medicine & 172 & 160\\
Math & 7688 & 1016 & Security & 100& 100\\
\bottomrule
\end{tabular}}
\captionof{table}{The statistical result of the original (Orig.)and mimicked (Mimic) ten subtasks from BIG-Bench and MMLU. For time and cost consideration, we limited the number of the generated samples on Math.}
\label{table: mimic data}
\end{minipage}
\hfill
\begin{minipage}[htb]{0.40\textwidth}
\small
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|c|c|c|c}
% \toprule
% \textbf{Setting} & \textbf{Fluency} & \textbf{Coherence} & \textbf{Answer} & \textbf{Category} \\
% \midrule
% Mimicking & 94.7 / 95.7 & 94.4 / 94.0 & 86.7 / 82.8 & - \\
% \midrule
% Extending & 98.3 / 100 & 96.7 / 96.7 & 92.7 / 82.0 &98.3 /100 \\
% \bottomrule
% \end{tabular}}
\begin{tabular}{l|c|c}
\toprule \textbf{Metrics} & \textbf{Mimicking} &\textbf{Extending} \\
\midrule 
Fluency & 94.7 / 95.7 & 98.3 / 100\\
Coherence & 94.4 / 94.0 & 96.7 / 96.7\\
Answer & 86.7 / 82.8 & 92.7 / 82.0\\
Category &  - & 98.3 / 100\\
\bottomrule
\end{tabular}}
\captionof{table}{The overview of Human Evaluation.The Scores are shown as full score rate (\%), with numbers after the slash indicating agreement rates (\%) among the five evaluators. }
\label{tab: human_evaluation}

\end{minipage}
\vspace{-3mm}
\end{figure}
For the extending strategy, we chose the dataset Sports, Algorithms (Algos), Algebra, and Physics (Phys), because the mimicking strategy performs poorly for benchmark leakage mitigation. For the Sports task, we extract the names of sports stars as seeds, recognizing that this task assesses the models' knowledge of these individuals. For the Algebra task, we extract key algebraic concepts as seeds. For Phys, we use GPT-4~\citep{GPT-4} to summarize the basic physical laws behind the original samples to use as seeds. Since the Algo task only encompasses a limited range of algorithmic topics, we employed GPT-4 to generate a list of 40 algorithm names. These names are then utilized as seeds for question generation. Based on these seeds, we utilize GPT-4 to generate new samples across multiple cognitive levels using extending prompts (details in Appendix~\ref{prompt appendix}). We manually maintain an equal distribution of the questions across each cognitive level. The static result is shown in Table~\ref{tab: containmation}.


\textbf{Human Evaluation.} To validate the reliability of our two strategies, we conduct a human evaluation involving five senior computational linguistics researchers, who have been trained in advance. For mimicked samples, evaluators review 120 randomly chosen samples, each including the question's category, the question, and the answer. They assess each question and answer paired based on three criteria: Fluency (the grammatical correctness and smoothness of the question), Coherence and Clarity (the logical clarity and explicit articulation of the question), and Accuracy of the Answer (the detailed evaluation guideline is shown in Appendix~\ref{appendix Mimiced Benchmark Evaluation Guideline}). In evaluating the extended samples, evaluators examine 60 randomly selected samples, which include the question, its cognitive level, and the reference answer. The assessment criteria are similar to those for the mimicked samples, with an additional focus on Category Accuracy (the detailed evaluation guideline is shown in Appendix~\ref{appendix: Extend Benchmark Evaluation Guideline}) to ensure that the question's cognitive level is appropriately identified. The human evaluation results, summarized in Table~\ref{tab: human_evaluation}, demonstrate high effectiveness and reliability of both strategies. 
% \begin{table}[ht]
% \centering
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{l|c|c|c|c}
% \toprule
% \textbf{Setting} & \textbf{Fluency} & \textbf{Coherence} & \textbf{Answer} & \textbf{Category} \\
% \midrule
% Mimicking & 94.7 / 95.7 & 94.4 / 94.0 & 86.7 / 82.8 & - \\
% \midrule
% Extending & 98.3 / 100 & 96.7 / 96.7 & 92.7 / 82.0 &98.3 /100 \\
% \bottomrule
% \end{tabular}}
% \caption{This table presents the overview of Human Evaluation. Results Scores are shown as full score rate (\%), with numbers after the slash indicating agreement rates (\%) among the five evaluators. }
% \label{tab: human_evaluation}

% \end{table}

\subsection{Evaluation Metric}\label{sec: evaluation}

 For mimicked samples, we adhere to the evaluation metrics used in the original tasks (details in Appendix~\ref{appendix detailed metric}). For extended samples, where questions are free-form, we adopt the ``LLM judgment'' methodology, following~\cite{zheng2023judging, bai2023benchmarking}. We give the question, reference answer (from updated sample) and the candidate's answer to LLMs to evaluate the answer across three dimensions: 1. \textbf{Accuracy:} evaluates the correctness of the answer, 2. \textbf{Coherence:} assesses the logical flow, and 3. \textbf{Factuality:} assessing the presence of factual errors (the evaluation prompt is shown in Appendix~\ref{prompt appendix}). We use the full-mark rate over the three dimensions as the metric and manually evaluate the "LLM judgment" result. The consistency of the model's results with human judgment achieved 90.8\% (detailed evaluation guideline is in Appendix~\ref{appendix: Extend Benchmark Evaluation Guideline} and detailed human evaluation result is shown in Table~\ref{tab: human_evaluation all}).

==> chapters/exp_bak.tex <==
\section{Experiment}\label{section experiment}


% \yixin{Section baseline}
\vspace{-1mm}
\subsection{Baseline}
To empirically validate the reliability of our auto-dataset update framework, we conducted experiments using seven
% public 
open source models: Llama-2-7b-chat, Llama-2-13b-chat~\cite{llama2}, Llama-3-8b-Instruction~\cite{llama3}, Mistral-7B-Instruct-v0.2, Mixtral-8x7B-Instruct-v0.1~\cite{mixtral-moe}, Yi-6b-chat, Yi-34b-chat~\cite{Yi}, and four closed-source models: GTP-4, ChatGPT, Claude2~\cite{claude2.1}, Gemini-pro~\cite{gemini}.

% \subsection{Is mimic method stable?}
\subsection{Evaluating the Stability of Updated Datasets} \label{sec: stable evaluation}
\vspace{-3mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htp]
\centering
     \includegraphics[scale=0.51]{figures/mimic_bbh_v2.pdf}
     \vspace{-2mm}
    \caption{Performance (\%) of the 11 involved models (zero-shot) on the original and mimicked (footnote $m$) Big-Bench. The generation of the mimicked dataset is conducted four times, the figure displays the average performance and standard deviation. Detailed results are shown in Table~\ref{tab: mimic result} }
     \label{fig: mimic different bbh}
\vspace{-5mm}
\end{figure*}
\begin{figure*}[htp]
\centering
     \includegraphics[scale=0.51]{figures/mimic_mmlu_v2.pdf}
      \vspace{-2mm}
    \caption{Performance (\%) of the 11 involved models (zero-shot) on the original and mimicked MMLU datasets. More detailed results are presented in Table~\ref{tab: mimic result mmlu} }
    \label{fig: mimic different mmlu}
    \vspace{-4mm}
\end{figure*}
Our proposed strategies are able to update datasets with minimum human effort whenever needed. That is, if we apply our strategy to the same dataset several times, we will obtain multiple different datasets. Clearly, a major concern is whether they can produce consistent evaluation results. To answer the above stability question, we choose the mimicking strategy and iterate the update process four times. Similar experiments under the extending strategy will be discussed in Section~\ref{sec: extending}. The statistical details can be found in Table~\ref{table: mimic data all}.
Based on four mimicked datasets, we calculate the average performance and the standard deviation of 11 baseline models under zero-shot in context learning (ICL). As shown in Figure~\ref{fig: mimic different bbh} and Figure~\ref{fig: mimic different mmlu} (more detail is shown in Table~\ref{tab: mimic result} and Table~\ref{tab: mimic result mmlu})
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It is apparent that: \textbf{1)} Compared with the performance of baselines on original datasets, their performance on our curated datasets are similar --- the difference of the two scores is 5\% on average except Element (we will discuss it later)
, 18\% max and 0\% min. 
This is mainly because the mimicked dataset has a similar style and difficulty; \textbf{2)} Among four different mimicked datasets, the standard deviation is limited, ranging from 0\% to 3\%. This demonstrates the stability of our mimicking dataset update strategy; \textbf{3)} The performance on the ``Periodic Elements'' in the mimicked dataset is markedly lower than in the original. This discrepancy can be attributed to the inclusion of the periodic table in the task description to assist the model in generating new questions. Unlike the original task, which exhaustively covered all possible one-hop questions like \textit{``What element contains one more proton than hydrogen?''}, the model, with the aid of the periodic table, generated more complex queries such as \textit{``What element contains two more protons than hydrogen?''}, which may need a reasoning step to answer compared to the original sample.
This also demonstrates the possibility of introducing external knowledge for updates, which will be future work.
\vspace{-2mm}
\subsection{Can mimicked datasets alleviate overestimation when benchmark leakage occurs?}\label{Sec: how data leakage affect}
\begin{table*}[htb]
\vspace{-3mm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc|cc|cc|cc|cc}
\toprule
\textbf{Model} &\textbf{Training} &\textbf{LoRA Only} &\textbf{Sports$_o$} &\textbf{Sports$_m$}& \textbf{Element$_o$} &\textbf{Element$_m$}& \textbf{Algos$_o$} 
&\textbf{Algos$_m$}
% & \textbf{conflict$_o$} &\textbf{conflict$_m$}
& \textbf{Phys$_o$} &\textbf{Phys$_m$}& \textbf{Math$_o$} &\textbf{Math$_m$}\\
\midrule
Llama-7b & None & - &94.3 & 94.2 & 19.9 & 3.1 & 2.0 & 2.6
% & 63.6 & 70.2 $\pm$ 0.4 
& 44.4 & 57.5  & 14.6 & 15.1 \\
Llama2-7b & + leakage & \checkmark & \cellcolor{extremelylightred} 99.7 & \cellcolor{medblue} 87.4 & \cellcolor{lightred} 57.1 & \cellcolor{medblue} 0.9 & \cellcolor{lightred} 42.2 & \cellcolor{lightred} 34.0 & \cellcolor{lightred} 74.9 & \cellcolor{medblue} 51.3 & \cellcolor{verylightred} 43.6 & \cellcolor{lightblue} 18.0 \\
Llama2-7b & + w rationale & \checkmark & \cellcolor{medblue} 92.4 & \cellcolor{medblue} 92.7 & \cellcolor{verylightred} 39.9 & \cellcolor{medblue} 1.3 & \cellcolor{lightred} 37.2 & \cellcolor{lightred} 36.0 & \cellcolor{verylightred} 67.9 & \cellcolor{lightblue} 57.5 & \cellcolor{verylightred} 25.8 & \cellcolor{lightblue} 19.8 \\
Llama2-7b & + leakage & \ding{55} & \cellcolor{extremelylightred} 99.8 & \cellcolor{medblue} 85.8 & \cellcolor{verylightred} 42.9 & \cellcolor{medblue} 0.0 & \cellcolor{lightred} 32.5 & \cellcolor{verylightred} 25.3 & \cellcolor{verylightred} 70.4 & \cellcolor{medblue} 52.5 & \cellcolor{verylightred} 42.0 & \cellcolor{lightblue} 19.2 \\
Llama2-7b & + w rationale & \ding{55} & \cellcolor{extremelylightred} 99.7 & \cellcolor{medblue} 88.7 & \cellcolor{verylightred} 47.8 & \cellcolor{medblue} 0.2 & \cellcolor{lightred} 40.6 & \cellcolor{lightred} 34.0 & \cellcolor{verylightred} 70.4 & \cellcolor{medblue} 55.6 & \cellcolor{verylightred} 32.4 & \cellcolor{extremelylightred} 20.8 \\
\midrule
Llama2-13b & None & - & 92.7 & 96.1 & 27.8 & 4.0 & 6.1 & 3.4  
% & 62.0 & 68.1
& 54.3 & 58.5 & 19.6 & 24.6  \\
Llama2-13b & + leakage & \checkmark & \cellcolor{extremelylightred} 99.8 & \cellcolor{medblue} 89.2 &  \cellcolor{lightred} 65.7 & \cellcolor{medblue} 1.1 & \cellcolor{lightred} 54.4 & \cellcolor{lightred} 42.7 & \cellcolor{verylightred} 83.9 & \cellcolor{lightblue} 61.3 & \cellcolor{verylightred} 43.6 & \cellcolor{medblue} 23.1 \\
Llama2-13b&  + w rationale & \checkmark  & \cellcolor{lightblue} 96.5 & \cellcolor{medblue} 91.7 & \cellcolor{verylightred} 49.3 & \cellcolor{medblue} 1.8 & \cellcolor{lightred} 45.6 & \cellcolor{lightred} 43.3 & \cellcolor{verylightred} 74.0 & \cellcolor{medblue} 55.0 & \cellcolor{verylightred} 32.0 & \cellcolor{lightblue} 28.6 \\
Llama2-13b& +leakage & \ding{55} & \cellcolor{extremelylightred} 99.7 & \cellcolor{medblue} 88.5 & \cellcolor{verylightred} 40.7 & \cellcolor{medblue} 0.0 & \cellcolor{lightred} 36.3 & \cellcolor{verylightred} 28.0 & \cellcolor{verylightred} 71.6 & \cellcolor{medblue} 45.0 & \cellcolor{verylightred} 42.3 & \cellcolor{lightblue} 26.4 \\
Llama2-13b& + w rationale & \ding{55} & \cellcolor{lightblue} 94.3 & \cellcolor{medblue} 88.9 & \cellcolor{verylightred} 43.6 & \cellcolor{medblue} 0.9 & \cellcolor{lightred} 37.3 & \cellcolor{lightred} 39.4 & \cellcolor{verylightred} 76.6 & \cellcolor{lightblue} 62.5 & \cellcolor{verylightred} 36.4 & \cellcolor{lightblue} 28.2 \\

\midrule
Llama2-8b & None & - & 98.2 & 99.7 & 36.9 & 3.3 & 4.1 & 6.0 & 70.4 & 67.5 & 43.9 & 34.8 \\
Llama3-8b & + leakage & \checkmark & \cellcolor{lightblue}98.7 & \cellcolor{medblue}92.5 & \cellcolor{verylightred}66.2 & \cellcolor{medblue}2.6 & \cellcolor{lightred}36.6 & \cellcolor{lightred}39.3 & \cellcolor{extremelylightred}77.8 & \cellcolor{lightblue}67.5 & \cellcolor{verylightred}57.1 & \cellcolor{medblue}34.4 \\
Llama3-8b & + w rationale & \checkmark & \cellcolor{medblue}98.1 & \cellcolor{medblue}87.7 & \cellcolor{lightred}68.2 & \cellcolor{lightblue}7.5 & \cellcolor{lightred}39.4 & \cellcolor{lightred}44.0 & \cellcolor{verylightred}86.9 & \cellcolor{lightblue}71.3 & \cellcolor{extremelylightred}51.5 & \cellcolor{lightblue}37.1 \\
Llama3-8b & + w rationale & \ding{55} & \cellcolor{medblue}93.2 & \cellcolor{medblue}85.6 & \cellcolor{verylightred}60.8 & \cellcolor{extremelylightred}12.4 & \cellcolor{lightred}36.6 & \cellcolor{lightred}39.3 & \cellcolor{extremelylightred}79.0 & \cellcolor{medblue}66.3 & \cellcolor{lightblue}44.5 & \cellcolor{medblue}29.9 \\
\midrule
Mistral-7b & None & - &88.8 & 94.0 & 27.1 & 5.3 & 15.7 & 20.0 & 53.1 & 57.5 & 12.5 & 25.8 \\
Mistral-7b & + leakage & \checkmark & \cellcolor{verylightred}99.8 & \cellcolor{medblue}87.7 & \cellcolor{extremelylightred}36.6 & \cellcolor{medblue}1.6 & \cellcolor{verylightred}38.1 & \cellcolor{verylightred}30.7 & \cellcolor{verylightred}66.7 & \cellcolor{lightblue}58.8 & \cellcolor{lightred}49.9 & \cellcolor{medblue}24.1 \\
Mistral-7b & + w rationale & \checkmark & \cellcolor{extremelylightred}95.0 & \cellcolor{medblue}90.4 & \cellcolor{verylightred}54.8 & \cellcolor{medblue}1.6 & \cellcolor{lightred}46.6 & \cellcolor{verylightred}40.6 & \cellcolor{verylightred}81.0 & \cellcolor{lightblue}58.8 & \cellcolor{verylightred}34.4 & \cellcolor{medblue}21.5 \\
Mistral-7b & + w rationale & \ding{55} & \cellcolor{extremelylightred}98.3 & \cellcolor{medblue}88.2 & \cellcolor{lightred}61.0 & \cellcolor{medblue}0.0 & \cellcolor{lightred}45.9 & \cellcolor{verylightred}38.0 & \cellcolor{lightred}88.9 & \cellcolor{medblue}56.8 & \cellcolor{lightred}48.0 & \cellcolor{lightblue}27.5 \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{Finetune performance (\%) (zero-shot) of Llama-2-7b-chat, Llama-2-13b-chat, Llama-3-8b-Instruction and Mistral-7B-Instruct on the original and mimicked BIG-bench examples (here we use the dataset from one of the iterations for time and cost consideration), \textit{leakage} denote using test prompt and the test set during training. \textit{w rationale} denote using test set with rational (Sec~\ref{Sec: how data leakage affect}). For our fine-tuning process, we specifically employed: full parameter and LoRA-only. Cells are blue if finetuning boosts the performance less than 5\% else are in red. Specifically, \uniformbox{CBE1EE}{0.2cm}{less than 0\%},  \uniformbox{E4F0F7}{0.2cm}{more than 0 \% but less than 5\%}, \uniformbox{FCF4EF}{0.2cm}{more than 5 \% but less than 10\%}, \uniformbox{F5E1D9}{0.2cm}{more than 10 \%}.} 
\label{tab: data leakge affect}
\vspace{-2mm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htb]
 \vspace{-2mm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc|cc|cc|cc|cc}
\toprule
\textbf{Model} &\textbf{Training} & \textbf{LoRA Only}& \textbf{Algebra$_o$} &\textbf{Algebra$_m$}& \textbf{Law$_o$} &\textbf{Law$_m$}& \textbf{Econ$_o$} 
&\textbf{Econ$_m$} & \textbf{Medicine$_o$} &\textbf{Medicine$_m$}& \textbf{Security$_o$} &\textbf{Security$_m$}\\
 
\midrule
Llama2-7b & None & - &14.0 & 17.2 & 57.8 & 70.0 & 28.1 & 32.7 & 41.9 & 49.8 & 58.0 & 60.0 \\
Llama2-7b & + leakage & \checkmark & \cellcolor{lightred} 52.0 & \cellcolor{verylightred} 31.2 & \cellcolor{lightred} 95.9 & \cellcolor{lightblue} 70.8 & \cellcolor{lightred} 65.8 & \cellcolor{lightblue} 34.6 & \cellcolor{lightred} 79.8 & \cellcolor{lightblue} 50.4 & \cellcolor{verylightred} 86.0 & \cellcolor{extremelylightred} 66.0 \\
Llama2-7b & + w rationale & \checkmark & \cellcolor{verylightred} 33.0 & \cellcolor{verylightred} 30.1 & \cellcolor{verylightred} 74.4 & \cellcolor{lightblue} 72.7 & \cellcolor{verylightred} 38.6 & \cellcolor{medblue} 31.7 & \cellcolor{verylightred} 53.8 & \cellcolor{lightblue} 50.8 & \cellcolor{extremelylightred} 67.0 & \cellcolor{lightblue} 60.0 \\
Llama2-7b & + leakage & \ding{55} & \cellcolor{lightred} 49.0 & \cellcolor{extremelylightred} 23.7 & \cellcolor{lightred} 93.4 & \cellcolor{lightblue} 70.9 & \cellcolor{lightred} 65.8 & \cellcolor{lightblue} 33.6 & \cellcolor{lightred} 79.2 & \cellcolor{lightblue} 51.1 & \cellcolor{verylightred} 84.0 & \cellcolor{lightblue} 60.0 \\
Llama2-7b & + w rationale & \ding{55} & \cellcolor{verylightred} 42.0 & \cellcolor{verylightred} 31.2 & \cellcolor{verylightred} 81.8 & \cellcolor{lightblue} 73.5 & \cellcolor{verylightred} 46.5 & \cellcolor{lightblue} 36.6 & \cellcolor{verylightred} 62.4 & \cellcolor{extremelylightred} 55.0 & \cellcolor{verylightred} 76.0 & \cellcolor{lightblue} 63.0 \\
\midrule
Llama2-13b & None & - &31.0 & 29.0 & 70.0 & 77.8 & 30.0 & 36.7 & 43.6 & 50.1 & 65.0 & 72.0 \\
Llama2-13b & +leakage & \checkmark & \cellcolor{verylightred} 51.0 & \cellcolor{lightblue} 30.1 & \cellcolor{lightred} 96.7 & \cellcolor{lightblue} 79.5 & \cellcolor{lightred} 67.5 & \cellcolor{extremelylightred} 42.5 & \cellcolor{lightred} 83.2 & \cellcolor{lightblue} 54.9 & \cellcolor{lightred} 92.0 & \cellcolor{lightblue} 76.0\\
Llama2-13b & + w rationale & \checkmark & \cellcolor{lightblue} 34.0 & \cellcolor{lightblue} 32.6 & \cellcolor{verylightred} 86.0 & \cellcolor{lightblue} 80.5 & \cellcolor{extremelylightred} 39.5 & \cellcolor{lightblue} 40.2 & \cellcolor{verylightred} 58.4 & \cellcolor{extremelylightred} 55.5 & \cellcolor{verylightred} 75.0 & \cellcolor{lightblue} 74.0\\
Llama2-13b & +leakage & \ding{55} & \cellcolor{verylightred} 48.0 & \cellcolor{medblue} 23.7 & \cellcolor{verylightred} 92.6 & \cellcolor{medblue} 70.9 & \cellcolor{lightred} 60.5 & \cellcolor{medblue} 36.6 & \cellcolor{lightred} 82.1 & \cellcolor{lightblue} 50.4 & \cellcolor{verylightred} 83.0 & \cellcolor{medblue} 71.0\\
Llama2-13b & + w rationale & \ding{55} & \cellcolor{extremelylightred} 38.0 & \cellcolor{extremelylightred} 35.4 & \cellcolor{verylightred} 86.7 & \cellcolor{lightblue} 80.1 & \cellcolor{verylightred} 50.0 & \cellcolor{lightblue} 40.5 & \cellcolor{verylightred} 65.3 & \cellcolor{extremelylightred} 55.6 & \cellcolor{verylightred} 79.0 & \cellcolor{lightblue} 74.0\\

\midrule
Llama3-8b & None & - &34.0 & 36.5 & 76.9 & 82.0 & 50.9 & 59.4 & 65.9 & 70.3 & 74.0 & 81.0 \\
Llama3-8b   & +leakage       & \checkmark & \cellcolor{verylightred}49.0 & \cellcolor{medblue}29.0 & \cellcolor{verylightred}92.6 & \cellcolor{lightblue}83.7 & \cellcolor{verylightred}72.8 & \cellcolor{lightblue}61.3 & \cellcolor{verylightred}87.2 & \cellcolor{lightblue}75.0 & \cellcolor{verylightred}89.0 & \cellcolor{medblue}80.0 \\
Llama3-8b   & + w rationale  & \checkmark & \cellcolor{verylightred}48.0 & \cellcolor{lightblue}38.7 & \cellcolor{verylightred}88.4 & \cellcolor{lightblue}83.7 & \cellcolor{verylightred}65.8 & \cellcolor{lightblue}63.4 & \cellcolor{extremelylightred}74.6 & \cellcolor{lightblue}71.8 & \cellcolor{verylightred}88.0 & \cellcolor{lightblue}84.0 \\
Llama3-8b   & + w rationale  & \ding{55}  & \cellcolor{verylightred}54.0 & \cellcolor{lightblue}39.7 & \cellcolor{verylightred}90.1 & \cellcolor{extremelylightred}87.2 & \cellcolor{verylightred}74.6 & \cellcolor{lightblue}61.3 & \cellcolor{verylightred}76.3 & \cellcolor{extremelylightred}75.6 & \cellcolor{extremelylightred}80.0 & \cellcolor{lightblue}83.0 \\
\midrule
Mistral-7b & None & - & 34.0 & 26.8 & 70.2 & 77.1 & 36.9 & 45.7 & 59.5 & 59.3 & 70.0 & 74.0 \\
Mistral-7b & + leakage & \checkmark & \cellcolor{verylightred} 63.0 & \cellcolor{extremelylightred} 32.6 & \cellcolor{verylightred} 96.7 & \cellcolor{medblue} 75.2 & \cellcolor{lightred} 70.2 & \cellcolor{medblue} 42.6 & \cellcolor{lightred} 90.2 & \cellcolor{medblue} 56.3 & \cellcolor{verylightred} 90.0 & \cellcolor{lightblue} 75.0 \\
Mistral-7b & + w rationale & \checkmark & \cellcolor{extremelylightred} 39.0 & \cellcolor{lightblue} 30.1 & \cellcolor{verylightred} 90.0 & \cellcolor{lightblue} 79.3 & \cellcolor{verylightred} 54.4 & \cellcolor{lightblue} 46.5 & \cellcolor{verylightred} 75.7 & \cellcolor{lightblue} 61.8 & \cellcolor{extremelylightred} 78.0 & \cellcolor{lightblue} 76.0 \\
Mistral-7b & + w rationale & \ding{55} & \cellcolor{verylightred} 50.0 & \cellcolor{lightblue} 26.9 & \cellcolor{verylightred} 97.5 & \cellcolor{lightblue} 80.1 & \cellcolor{lightred} 68.4 & \cellcolor{extremelylightred} 50.8 & \cellcolor{verylightred} 79.8 & \cellcolor{lightblue} 62.1 & \cellcolor{verylightred} 86.0 & \cellcolor{lightblue} 76.0 \\

\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Finetune performance (\%) of Llama-2-7b-chat, Llama-2-13b-chat, Llama-3-8b-Instruction and Mistral-7B-Instruct on the mimicked MMLU examples. Following the setting in Table~\ref{tab: data leakge affect}.}
\label{tab: data leakge affect mmlu}
\vspace{-2mm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% One of our main motivations is to automate dataset updates, so as to mitigate the overestimation caused by benchmark leakage issues toward reliable evaluation.  To validate the benchmark leakage issue, we finetune models using the testing data from original datasets (combined into one testing set) and evaluate them on our updated dataset to see if the performance is affected similarly or not. 
One of our main motivations is to automate dataset updates toward reliable evaluation. In this section, we validate how our approach mitigates the overestimation caused by benchmark leakage issues.
% We exclusively utilize a supervised fine-tuning (SFT) training setting, as data leakage during a model's pretraining phase can typically be detected by current contamination detection methods~\cite{shi2023detecting}. In contrast, our experiment demonstrates that when data leakage happened occurring during the SFT stage can not be effectively detected by cureent methods (detailed results of this investigation are provided in Appendix~\ref{appendix: Contamination Detection for the Finetuned Models}).  
 We choose four baseline models, Llama-2-7b-chat, Llama-2-13b-chat~\cite{llama2}, Llama-3-8b-Instruction~\cite{llama3} and Mistral-7B-Instruct~\cite{mistral-7b}, and follow the training configuration in previous work~\cite{zhou2023don, llama2, xu2023wizardlm} for fair evaluation (detailed configuration is in the Appendix~\ref{model setting appendix}). For each model, there are three training settings: \textbf{1)} \textit{None}, which denotes the original model; \textbf{2)} \textit{leakage}, referring to the finetuned model using the above leakage simulation; \textbf{3)} \textit{w rationale}, which included rationales for each leakage sample during finetuning. Thus, these rationale finetuning will also improve the models' reasoning ability over the testing samples. In specific, we follow~\cite{wei2022finetuned} to generate rationales using GPT-4~\cite{GPT-4} for the correct choice. The detailed prompt is shown in the Appendix~\ref{ration creation}.
As shown in Table~\ref{tab: data leakge affect} and Table~\ref{tab: data leakge affect mmlu}, we find that: \textbf{1)} on the original dataset, the performance of all leakage simulations increases dramatically, no matter finetune via LoRA~\cite{hu2021lora} or not. This is consistent with previous works~\cite{zhou2023don}, showing the serious overestimation issue; \textbf{2)} on our mimicked datasets, the performance of all leakage simulations generally decreases or remains similar, except task Algos, and Algebra (will be discussed with the extending strategy Section~\ref{sec: extending}); \textbf{3)} in most cases, the performance of \textit{leakage} setting is better than that of \textit{w rationale} on original datasets, while the results are opposite in mimicked datasets. We attribute this to the improvement of the generalization ability through training with rationales, which will mitigate the overfitting performance of \textit{leakage}/\textit{w rationale}, aligning with~\cite{longpre2023flan}. 
\textbf{4)} Llama-2-13b gets improved from 3.4\% to 43.3\% on the task Algos after finetuning. We hypothesize this enhancement is attributable to model learning the distribution of labels, considering that the labels range uniformly from 1 to 10. This indicates a limitation of the mimicking strategy: the possibility of benchmark leakage leading to models learning from the answer distribution, which in turn leads to an overestimated performance.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\vspace{-3mm}
\subsection{Extending Strategy: Stability \& Dealing with benchmark Leakage }\label{sec: extending}
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2mm}
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcc|c|c}
\toprule 
\textbf{Model} &  \textbf{Training} &\textbf{LoRA only} &\textbf{Algebra} & \textbf{Algos} \\
\midrule

Llama2-7b & None & -& \textbf{4.2} $\pm{0.6}$ & \textbf{10.2} $\pm{0.5}$ \\
Llama2-7b & + leakage & \checkmark & 1.6 $\pm{0.6}$  & 2.2 $\pm{0.6}$\\
Llama2-7b & + w rationale & \checkmark& 1.2 $\pm{0.0}$ & 5.3 $\pm{0.5}$\\
Llama2-7b & + leakage & \ding{55} & 1.8 $\pm{0.6}$ &1.1 $\pm{0.0}$ \\
Llama2-7b & + w rationale & \ding{55} & 2.1 $\pm{0.5}$ & 8.9 $\pm{0.8}$\\
\midrule
Llama2-13b& None &-  & \textbf{8.5}  $\pm{0.4}$& \textbf{11.9} $\pm{0.8}$ \\
Llama2-13b& + leakage & \checkmark& 6.6 $\pm{0.5}$ & 5.1 $\pm{0.1}$\\
Llama2-13b&  + w rationale& \checkmark & 6.4 $\pm{0.9}$& 11.2 $\pm{0.8}$\\
Llama2-13b& + leakage & \ding{55} & 1.5 $\pm{0.4}$& 0.5 $\pm{0.4}$\\
Llama2-13b&  + w rationale& \ding{55} & 5.7 $\pm{0.5}$& 7.7 $\pm{1.2}$\\
\midrule
Llama3-8b& None &-  & \textbf{34.6}  $\pm{1.6}$& \textbf{46.7} $\pm{2.1}$ \\
Llama3-8b& + leakage & \checkmark& 12.1 $\pm{0.5}$ & 21.3 $\pm{2.2}$\\
Llama3-8b&  + w rationale& \checkmark & 17.8 $\pm{1.3}$& 17.5 $\pm{1.8}$\\
Llama3-8b&  + w rationale& \ding{55} & 15.3 $\pm{1.6}$& 18.7 $\pm{1.2}$\\
% LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
\midrule
Mistral-7b & None & -& \textbf{21.8} $\pm{1.7}$  & \textbf{36.8} $\pm{0.0}$\\
Mistral-7b & + leakage & \checkmark & 0.9 $\pm{0.5}$ &  5.3 $\pm{0.5}$\\
Mistral-7b &  + w rationale& \checkmark  & 4.4 $\pm{0.6}$ &  9.1 $\pm{0.5}$\\
Mistral-7b &  + w rationale& \ding{55}  & 2.3 $\pm{0.2}$& 4.4 $\pm{0.8}$\\
\bottomrule
\end{tabular} }
\vspace{-2mm}
\captionof{table}{Average percentage (\%)  of full-mark of the fine-tuned model on the extended dataset over the four iterations.}
\label{tab: data leakage extend}
\vspace{-5mm}
\end{wrapfigure}
As shown in Section~\ref{Sec: how data leakage affect}, the mimicking strategy does not work well on two datasets: Algos and Algebra. The benchmark leakage issue still leads to a severe overestimation of the model, which we will further explore using the extending strategy in this section. Following the experiment settings of the mimicking strategy, we leverage the same baseline models with leakage simulations, as well as four iterations of dataset updates for stability verification (updating process defined in Section~\ref{Extend setting} and Section~\ref{sec: Updated Dataset Analysis} and statistical details can be found in Table~\ref{table: extend data all}). As shown in Table~\ref{tab: data leakage extend}, the standard deviation among four runs is quite low, demonstrating the stability of our extending strategy. This is not surprising as extending strategy can be regarded as an extension of the mimicking strategy with varying cognitive levels for controllable difficulty (Section~\ref{sec diff}). 
To investigate the effectiveness, we employ baseline models in the mimicking strategy that are fine-tuned on test samples from the original datasets. Table~\ref{tab: data leakage extend} shows that all performances of leakage simulations greatly decrease compared with original models due to the overfitting issue. Moreover, the decline of \textit{leakage} is more than that of \textit{w rationale} because it is alleviated through the improved generalization ability via learning with rationales. However, note that even with rationales, the model still exhibits signs of overfitting, which may improve its performance on the original test set. 

% \subsection{Can we control the question difficulty using the extend setting?} \label{sec diff}
\vspace{-3mm}
\subsection{Is it possible to control the sample difficulty using the Extending Strategy?} \label{sec diff}
\begin{figure}[htb]
\centering
\includegraphics[scale=0.20]{figures/extend_result_flat.pdf}
\vspace{-2mm}
    \caption{Rull-mark rate (\%) of GPT-4, ChatGPT, Claude, and Gemini on the extended Sports (a), Phys (b) dataset on different cognitive levels. Overall is the average score across the four levels.}
    \label{fig: extend result}  
\vspace{-4mm}
\end{figure}

Except for overestimation leading by benchmark leakage in Section~\ref{sec: extending}, there is another issue on the task Sports and Phys (Table~\ref{tab: data leakge affect} and Table~\ref{tab: data leakge affect mmlu})  --- the absolute scores are notably high, suggesting that the questions are relatively simple and thus insufficient to differentiate the models (i.e., 3.82\% and 4.30\% difference on average for models GPT-4, ChatGPT, Gemini, and Claude). 
% In this section, we explore how to control the difficulty of extended datasets from two aspects: \textbf{1)} adjusting the cognitive levels, more abstract levels are expected to produce more difficult samples; and \textbf{2)} entity popularity, questions about long-tail entities are much more difficult to answer for LLMs~\cite{mallennot}. Specifically, we use the extracted sports star name and the summarized common physical law as the seed and update the dataset using extending strategy (Section~\ref{sec Updated Dataset Analysis}). We use models GPT-4, ChatGPT, Gemini, and Claude as the baseline for their indistinguishable performance.
In this section, we explore the feasibility of modulating the difficulty of the extended data samples to better discern and differentiate model capabilities. In our extension work, we start by abstracting the original question into core entities, statements, or adding additional knowledge, then use Bloom’s taxonomy to further extend. This naturally allows for the adjustment of question difficulty in two ways, as indicated by prior findings: 1) work~\cite{krathwohl2002revision} suggests that cognitive demand increases with higher cognitive processes. Accordingly, by adjusting to more abstract cognitive levels, we expect to produce more challenging samples; 2) work~\cite{mallennot} indicates that as the popularity of the subject entity increases, the difficulty of the question decreases. Thus, the popularity of the input seed could be strategically manipulated to adjust the complexity of the generated questions. To validate the efficacy of our framework in controlling difficulty, we use the extracted sports star name and the summarized common physical law as the seed to update the dataset using the extending strategy (Section~\ref{sec: Updated Dataset Analysis}). We use models GPT-4, ChatGPT, Gemini, and Claude as the baseline for their indistinguishable performance.
% \yixin{As shown in Figure~\ref{fig: extend result}, we can see }

As shown in Figure~\ref{fig: extend result}, \textbf{1)} on the extended Sports and Phys datasets, the four models' performance show larger variance (23.76\%, 14.04\% respectively), compared with it on original datasets; 
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-2mm}
\includegraphics[scale=0.28]{figures/pop.pdf} 
\vspace{-1mm}
\caption{Rull-mark rate (\%) of GPT-4, ChatGPT, Claude and Gemini on the extended ``sport understanding'' datasets on different popularity levels. We depict the number of questions on different popularity levels.}
\label{fig: pop result}
\vspace{-5mm}
\end{wrapfigure}
\textbf{2)} overall, samples test ``Apply'' and ``Evaluation'' cognitive levels are found to be more challenging. This finding indicates that manipulating the cognitive level in the extending strategy is an effective way of controlling the difficulty of the generated questions in our framework. It also highlights the importance of focusing on models' capabilities across different cognitive levels. Some models exhibit significant disparities in performance across various cognitive levels, while GPT-4  shows stronger performance. 
% \begin{figure}[htb]
% \centering
% \begin{minipage}[t]{0.48\textwidth}
% \includegraphics[scale=0.28]{figures/pop.pdf}
%     \caption{Rull-mark rate (\%) of GPT-4, ChatGPT, Claude and Gemini on the extended ``sport understanding'' datasets on different popularity levels. We depict the number of questions on different popularity levels.}
%     \label{fig: pop result} 
% \end{minipage}
% \begin{minipage}[t]{0.48\textwidth}
% \end{minipage}
% \end{figure} 

In addition to assessing how cognitive levels influence performance, we explored how the popularity of the seeds used in 
% question generation 
dataset update affects model performance. Following previous work~\cite{mallennot}, where using Wikipedia page views as the measure of popularity, we gather the total page views for each seed throughout the year 2023 and use it as the popularity. As shown in Figure~\ref{fig: pop result}, despite an uneven distribution of seed popularity in the extended dataset, a clear trend emerged: there was a noticeable increase in model performance when using more popular seeds to generate the question. 
This observation suggests that the popularity of the seed input can also be strategically manipulated to control the difficulty of the generated questions in our framework.
% \begin{figure}[ht]
% \begin{minipage}{0.50\textwidth}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|c|c|c}
% \toprule
% \textbf{Dataset} & \textbf{\#Total} & \textbf{\#Clean}& 
% \textbf{\#Input} 
% \textbf{Dirty}
%  &  \textbf{\#Input-label Dirty} \\  
% \midrule
% Algebra & 80& 80& 0 &0\\
% Algos & 320 & 320&0 &0 \\
% Phys & 80 & 79& 1 & 0\\
% Sports & 824 & 824& 0 &0\\
% \bottomrule
% \end{tabular}}
% % \begin{tabular}{l|c|c|c|c}
% % \toprule
% %  & \textbf{Algebra} & \textbf{Algos} & \textbf{Phys} & \textbf{Sports} \\
% % \midrule
% % \textbf{\#Total} & 80 & 320 & 80 & 824 \\
% % \textbf{\#Clean} & 80 & 320 & 79 & 824 \\
% % \textbf{\#Input Dirty} & 0 & 0 & 1 & 0 \\
% % \textbf{\#Input-label Dirty} & 0 & 0 & 0 & 0 \\
% % \bottomrule
% % \end{tabular}}

% \captionof{table}{The contamination report on the extended data samples. We compare the generated sample with the web source, the benchmark source, and IFT dataset.}
% \label{tab: containmation}
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\textwidth}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcc|c}
% \toprule 
% \textbf{Model} &  \textbf{Training} &\textbf{LoRa only} &\textbf{Algebra} \\
% \midrule

% Llama-7b & None & -& \textbf{26.3}  $\pm{1.6}$ \\

% Llama-7b & + w rationale & \checkmark & 8.9 $\pm {0.5}$ \\
% Llama-7b & + w rationale & \ding{55} & 22.1 $\pm {0.5}$ \\
% \midrule
% Llama-13b& None &-  & \textbf{33.9}  $\pm {1.9}$  \\
% Llama-13b&  + w rationale& \checkmark & 26.0 $\pm {1.0}$  \\
% Llama-13b&  + w rationale& \ding{55} & 9.7  $\pm {1.6}$ \\
% \midrule
% Llama3-8b& None &- & \textbf{59.0} $\pm {1.5}$\\
% Llama3-8b&  + w rationale& \checkmark & 39.6 $\pm {0.4}$  \\
% Llama3-8b&  + w rationale& \ding{55} & 41.1  $\pm {1.0}$ \\
% % LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
% \midrule
% Mistral-7b & None & -& \textbf{45.5} $\pm {0.4}$ \\
% Mistral-7b &  + w rationale& \checkmark   & 17.9 $\pm {0.4}$\\
% Mistral-7b &  + w rationale& \ding{55}  & 6.8 $\pm {2.2}$\\
% \bottomrule
% \end{tabular} 
% }
% \captionof{table}{Average percentage (\%)  of full-mark of the fine-tuned model on the extended dataset from Claude3 as examiner}
% \label{tab: data leakage extend claude3}
% \end{minipage}
% \end{figure}


 \subsection{Adaptable to Models Beyond the GPT Backbone}\label{sec: Adaptable to models beyond the GPT backbone}

% \begin{wrapfigure}{r}{0.35\textwidth}
%  \vspace{-6mm}
% \centering
% \resizebox{0.35\textwidth}{!}{%
% \begin{tabular}{lcc|c|c}
% \toprule 
% \textbf{Model} &  \textbf{Training} &\textbf{LoRA only} &\textbf{Algebra} \\
% \midrule

% Llama2-7b & None & -& \textbf{26.3}  $\pm{1.6}$ \\

% Llama2-7b & + w rationale & \checkmark & 8.9 $\pm {0.5}$ \\
% Llama2-7b & + w rationale & \ding{55} & 22.1 $\pm {0.5}$ \\
% \midrule
% Llama2-13b& None &-  & \textbf{33.9}  $\pm {1.9}$  \\
% Llama2-13b&  + w rationale& \checkmark & 26.0 $\pm {1.0}$  \\
% Llama2-13b&  + w rationale& \ding{55} & 9.7  $\pm {1.6}$ \\
% \midrule
% Llama3-8b& None &- & \textbf{59.0} $\pm {1.5}$\\
% Llama3-8b&  + w rationale& \checkmark & 39.6 $\pm {0.4}$  \\
% Llama3-8b&  + w rationale& \ding{55} & 41.1  $\pm {1.0}$ \\
% % LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
% \midrule
% Mistral-7b & None & -& \textbf{45.5} $\pm {0.4}$ \\
% Mistral-7b &  + w rationale& \checkmark   & 17.9 $\pm {0.4}$\\
% Mistral-7b &  + w rationale& \ding{55}  & 6.8 $\pm {2.2}$\\
% \bottomrule
% \end{tabular} }
% \captionof{table}{Average performance (\%) of the fine-tuned models on the extended datasets generated by Claude-3-Opus over the two iterations.}
% \label{tab: data leakage extend claude3}
% \end{wrapfigure}
Relying solely on GPT-4 may introduce biases, such as self-preference, particularly when employing the ``LLM-as-an-Examiner'' methodology~\cite{bai2023benchmarking}. In this section we expand the experimentation by using Claude-3-Opus~\citep{Claude-3} to generate new samples, demonstrating the framework's adaptability to other backbones. Thus by using multi-source data, helps mitigate the bias associated with exclusively using GPT-4.
Using Claude-3-Opus, we extend the algebra task, where the mimicking strategy is less effective, following the setting in Section~\ref{Sec: how data leakage affect}. Due to time and cost considerations, we only conduct the generation process two times, the static result is shown in Table~\ref{table: extend data all}.  We deploy models that are fine-tuned on test samples from the original datasets with rationales (\textit{w rationale}), which demonstrates superior performance compared to \textit{leakage} simulations to investigate the effectiveness. Shown in Table~\ref{tab: data leakage extend claude3}, the performance of the leakage simulations significantly declines compared to the original models, indicating the adaptability of our framework of using other models as backbone.
\begin{figure}[htb]
\vspace{-2mm}
\begin{minipage}[htb]{0.40\textwidth}
\small
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc|c}
\toprule 
\textbf{Model} &  \textbf{Training} &\textbf{LoRA only} &\textbf{Algebra} \\
\midrule

Llama2-7b & None & -& \textbf{26.3}  $\pm{1.6}$ \\

Llama2-7b & + w rationale & \checkmark & 8.9 $\pm {0.5}$ \\
Llama2-7b & + w rationale & \ding{55} & 22.1 $\pm {0.5}$ \\
\midrule
Llama2-13b& None &-  & \textbf{33.9}  $\pm {1.9}$  \\
Llama2-13b&  + w rationale& \checkmark & 26.0 $\pm {1.0}$  \\
Llama2-13b&  + w rationale& \ding{55} & 9.7  $\pm {1.6}$ \\
\midrule
Llama3-8b& None &- & \textbf{59.0} $\pm {1.5}$\\
Llama3-8b&  + w rationale& \checkmark & 39.6 $\pm {0.4}$  \\
Llama3-8b&  + w rationale& \ding{55} & 41.1  $\pm {1.0}$ \\
% LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
\midrule
Mistral-7b & None & -& \textbf{45.5} $\pm {0.4}$ \\
Mistral-7b &  + w rationale& \checkmark   & 17.9 $\pm {0.4}$\\
Mistral-7b &  + w rationale& \ding{55}  & 6.8 $\pm {2.2}$\\
\bottomrule
\end{tabular} }
\captionof{table}{Average performance (\%) of the fine-tuned models on the extended datasets generated by Claude-3-Opus over the two iterations.}
\label{tab: data leakage extend claude3}
\end{minipage}
\hfill
\begin{minipage}[htb]{0.58\textwidth}
\small
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Dataset} & \textbf{\#Total} & \textbf{\#Clean}& 
\textbf{\#Input} 
\textbf{Dirty}
 &  \textbf{\#Input-label Dirty} \\  
\midrule
Algebra & 154 & 154& 0 &0\\
Algos & 320 & 320&0 &0 \\
Phys & 80 & 79& 1 & 0\\
Sports & 824 & 824& 0 &0\\
\bottomrule
\end{tabular}}
\captionof{table}{The contamination report on the extended data samples. We compare the generated sample with the web, benchmark, and IFT dataset source. It is important to note that of the samples in the Algebra task, 80 are generated by GPT-4, while the remainder are produced by Claude-3-Opus (detailed in Section~\ref{sec: Adaptable to models beyond the GPT backbone}). Considering the time and cost, we only use the first iteration, which statistics is shown in Table~\ref{table: extend data all}}
\label{tab: containmation}
\end{minipage}
\vspace{-5mm}
\end{figure}
\vspace{-3mm}
\subsection{Does the extended data sample have benchmark leakage problem?}\label{comtainmation report}
\vspace{-2mm}
If the generated samples are from some of the pre-trained datasets, it will lead to potential benchmark leakage problems. In this section, we measure the potential benchmark leakage in these extended 
% questions, 
samples\footnote{Considering the time and cost, we only use the first iteration, which statistics is shown in Table~\ref{table: extend data all})}.
Following previous work~\cite{li2023open, dodge2021documenting}, we calculate the similarity between newly generated data and data from public sources. We involve public data from three sources: web data, public benchmarks, and Instruction Fine-Tuning (IFT) data. For web data, we  extract relevant queries 
% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-2mm}
% \centering
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{l|c|c|c|c}
% \toprule
% \textbf{Dataset} & \textbf{\#Total} & \textbf{\#Clean}& 
% \textbf{\#Input} 
% \textbf{Dirty}
%  &  \textbf{\#Input-label Dirty} \\  
% \midrule
% Algebra & 154 & 154& 0 &0\\
% Algos & 320 & 320&0 &0 \\
% Phys & 80 & 79& 1 & 0\\
% Sports & 824 & 824& 0 &0\\
% \bottomrule
% \end{tabular}}
% \captionof{table}{The contamination report on the extended data samples. We compare the generated sample with the web, benchmark, and IFT dataset source.}
% \label{tab: containmation}
% \vspace{-3mm}
% \end{wrapfigure}
and context through Bing searches API, for public benchmarks we select several popular benchmarks: MMLU, HellaSwag~\cite{zellers2019hellaswag}, BIG-bench, ARC~\cite{clark2018think}, CommonsenseQA~\cite{commonsenseqa}, Winogrande~\cite{sakaguchi2021winogrande}, and for IFT dataset we select LaMini-Instruction~\citep{lamini-lm}, WizardLM-evol-instruct-V2~\cite{xu2023wizardlm}, and P3~\cite{sanh2021multitask}.
Following the methodology in \cite{li2023open}, we utilize Meteor \cite{meteor} as our similarity metric, and use the same parameter setting in \cite{li2023open}. We categorized the generated samples following~\cite{dodge2021documenting}:
\textbf{Clean:} No contamination present. \textbf{Input Dirty:} Only the question appears in the public data. \textbf{Input-and-Label Dirty:} Both question and answer are found in the public data. As evidenced in Table~\ref{tab: containmation}, extending strategy won't have benchmark leakage issue.


% \begin{table}[htbp]
% \centering
% \caption{Aligning around the $\pm$ symbol}
% \begin{tabular}{lccR{0.2cm}@{$\pm$}L{1.2cm}R{1.2cm}@{$\pm$}L{1.2cm}}
% \toprule
% \textbf{Model} & \textbf{Training} & \textbf{LoRa only} & \multicolumn{2}{c}{\textbf{Algebra}} & \multicolumn{2}{c}{\textbf{Algos}} \\
% \midrule
% Llama-7b    & None         & -          & 4.2 & 0.6 & 10.2 & 0.5 \\
% Llama-7b    & + leakage    & \checkmark & 1.6 & 0.6 &  2.2 & 0.6 \\
% Llama-7b    & + w rationale& \checkmark & 1.2 & 0.0 &  5.3 & 0.5 \\
% Llama-7b    & + leakage    & \ding{55}  & 1.8 & 0.6 &  1.1 & 0.0 \\
% Llama-7b    & + w rationale& \ding{55}  & 2.1 & 0.5 &  8.9 & 0.8 \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{wrapfigure}{r}{0.5\textwidth}
% \centering
% \caption{Aligning around the $\pm$ symbol}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcc|R{0.8cm}@{$\pm$}L{0.8cm}R{0.8cm}@{$\pm$}L{0.8cm}}
% \toprule
% \textbf{Model} & \textbf{Training} & \textbf{LoRa only} & \multicolumn{2}{c}{\textbf{Algebra}} & \multicolumn{2}{c}{\textbf{Algos}} \\
% \midrule
% Llama-7b    & None         & -          & 4.2 & 0.6 & 10.2 & 0.5 \\
% Llama-7b    & + leakage    & \checkmark & 1.6 & 0.6 &  2.2 & 0.6 \\
% Llama-7b    & + w rationale& \checkmark & 1.2 & 0.0 &  5.3 & 0.5 \\
% Llama-7b    & + leakage    & \ding{55}  & 1.8 & 0.6 &  1.1 & 0.0 \\
% Llama-7b    & + w rationale& \ding{55}  & 2.1 & 0.5 &  8.9 & 0.8 \\
% \bottomrule
% \end{tabular}}
% \end{wrapfigure}



==> chapters/exp_v1.tex <==
\section{Experiment}\label{section experiment}


% \yixin{Section baseline}
\vspace{-1mm}
\subsection{Baseline}
To empirically validate the reliability of our auto-dataset update framework, we conducted experiments using seven
% public 
open source models: Llama-2-7b-chat, Llama-2-13b-chat~\cite{llama2}, Llama-3-8b-Instruction~\cite{llama3}, Mistral-7B-Instruct-v0.2, Mixtral-8x7B-Instruct-v0.1~\cite{mixtral-moe}, Yi-6b-chat, Yi-34b-chat~\cite{Yi}, and four closed-source models: GTP-4, ChatGPT, Claude2~\cite{claude2.1}, Gemini-pro~\cite{gemini}.

% \subsection{Is mimic method stable?}
\subsection{Evaluating the Stability of Updated Datasets} \label{sec: stable evaluation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our proposed strategies are able to update datasets with minimum human effort whenever needed. That is, if we apply our strategy to the same dataset several times, we will obtain multiple different datasets. Clearly, a major concern is whether they can produce consistent evaluation results. To answer the above stability question, we choose the mimicking strategy and iterate the update process four times. Similar experiments under the extending strategy will be discussed in Section~\ref{sec: extending}. The statistical details can be found in Table~\ref{table: mimic data all}.
Based on four mimicked datasets, we calculate the average performance and the standard deviation of 11 baseline models under zero-shot in context learning (ICL). As shown in Figure~\ref{fig: mimic different bbh} and Figure~\ref{fig: mimic different mmlu} (more detail is shown in Table~\ref{tab: mimic result} and Table~\ref{tab: mimic result mmlu})
\begin{figure*}[htb]
\centering
     \includegraphics[scale=0.51]{figures/mimic_bbh_v2.pdf}
    \caption{Performance (\%) of the 11 involved models (zero-shot) on the original and mimicked (footnote $m$) Big-Bench. The generation of the mimicked dataset is conducted four times, the figure displays the average performance and standard deviation. Detailed results are shown in Table~\ref{tab: mimic result} }
     \label{fig: mimic different bbh}
\end{figure*}

\begin{figure*}[htb]
\centering
     \includegraphics[scale=0.51]{figures/mimic_mmlu_v2.pdf}
    \caption{Performance (\%) of the 11 involved models (zero-shot) on the original and mimicked MMLU datasets. More detailed results are presented in Table~\ref{tab: mimic result mmlu} }
    \label{fig: mimic different mmlu}
    \vspace{-5mm}
\end{figure*}

% \begin{figure}[htb]
% \vspace{-3mm}
% \begin{minipage}{0.49\textwidth}
% \centering
%     \includegraphics[scale=0.51]{Styles/figures/mimic_bbh_var.pdf}
%     \label{figure: bbh_var}
% \caption{The standard deviation of performance across four iterations for the 11 involved models on mimicked Big-Bench. More detailed results are presented in Table~\ref{tab: mimic result} }
% \end{minipage}
% \hfill
% \begin{minipage}{0.49\textwidth}
% \centering
%     \includegraphics[scale=0.51]{Styles/figures/mimic_mmlu_var.pdf}
%     \label{figure: mmlu_var}
%     \caption{The standard deviation of performance across four iterations for the 11 involved models on mimicked MMLU. More detailed results are presented in Table~\ref{tab: mimic result mmlu} }
% \end{minipage}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[htb]
% \vspace{-2mm}
% \centering

% \resizebox{0.98\textwidth}{!}{%
% \begin{tabular}{lcc|cc|cc|cc|cc}
% \toprule
% \textbf{Model} & \textbf{Algebra$_o$} &\textbf{Algebra$_m$}& \textbf{Law$_o$} &\textbf{Law$_m$}& \textbf{Econ$_o$} 
% &\textbf{Econ$_m$} & \textbf{Medicine$_o$} &\textbf{Medicine$_m$}& \textbf{Security$_o$} &\textbf{Security$_m$}\\
% \midrule
% GPT-4    & 76.0 & 72.5 $\pm$ 1.6 & 89.7  & 91.6  $\pm$ 0.9 &       66.7 & 76.3 $\pm$ 2.3 &   
% % 63.2   & 62.1 $\pm$ 0.9 &
% 80.7& 85.2 $\pm$ 1.7 & 85.0 & 91.6 $\pm$ 0.2\\
% ChatGPT  & 39.0 &  37.7 $\pm$  0.1 & 73.6 & 80.6 $\pm$ 0.0 &   46.4 & 55.0 $\pm$ 2.4 &   
% % 70.7   & 74.1 $\pm$ 0.3 &
% 70.1 & 73.5 $\pm$ 0.2& 79.0 & 81.9 $\pm$ 0.2\\
% Gemini  & 35.0 & 36.6 $\pm$ 0.0  &  82.6 & 85.2  $\pm$ 0.0 &     54.4 & 57.4 $\pm$ 0.2 & 
% % 81.9  & 85.5 $\pm$ 0.4 &
% 69.3 & 71.5 $\pm$ 1.2 & 78.0 & 82.0 $\pm$ 0.0\\
% Claude2.1 & 47.0  & 52.6 $\pm$ 0.2 &  69.4  & 70.2  $\pm$ 0.1&   40.4 & 54.4  $\pm$ 0.2 &     
% % 65.0   & 73.2 $\pm$ 0.0  & 
% 60.7 & 62.5 $\pm$ 0.1&  
%  68.0 & 75.6 $\pm$ 2.4\\


% \midrule
% Llama-7b & 14.0 & 17.2 $\pm$ 0.2 & 57.8 & 68.0  $\pm$ 2.1& 28.1 & 32.3 $\pm$ 1.6 
% % & 63.6 & 70.2 $\pm$ 0.4 
% & 41.9 & 49.8 $\pm$ 1.4 & 58.0 & 60.6 $\pm$ 2.3\\
% Llama-13b & 31.0 & 29.0 $\pm$ 0.1 & 70.0 & 77.2 $\pm$ 0.2& 30.0 & 36.0 $\pm$ 1.6 
% % & 62.0 & 68.1 $\pm$ 0.8 
% &43.6  & 50.1 $\pm$ 1.2  & 65.0 & 72.0 $\pm$ 1.2 \\
% Llama3-8b & 34.0 & 35.5 $\pm$ 1.0 & 76.9 & 81.4 $\pm$ 0.6 &50.9 & 59.4 $\pm$ 0.0 &65.9 &70.2 $\pm$ 0.1& 74.0 & 81.4 $\pm$ 0.3\\
% Mistral-7b & 34.0 & 27.9 $\pm$ 1.0 & 70.2 & 77.1$\pm$ 0.2 & 36.9 & 45.7 $\pm$ 0.7 
% % & 80.1 & 83.2 $\pm$ 0.6 
% & 59.5 & 59.3 $\pm$ 0.1 & 70.0 & 74.4 $\pm$ 2.8\\
% Mistral-8x7b & 41.0 & 41.5 $\pm$ 0.4 & 74.4 & 77.9 $\pm$ 1.0 & 53.5 & 62.5 $\pm$ 0.2
% % & 78.1 & 77.0 $\pm$ 0.8 
% & 67.6 & 73.5 $\pm$ 1.2 & 74.0 & 77.1 $\pm$ 2.9\\
% Yi-6B & 27.0 & 26.7 $\pm$ 2.3 & 68.6 & 73.3 $\pm$ 0.2 & 33.3 & 43.6 $\pm$ 1.6 
% % & 66.6 &70.4 $\pm$ 0.5 
% & 65.9 & 61.9 $\pm$ 0.3 & 67.0 & 72.9 $\pm$ 2.1\\
% Yi-34B & 33.0 & 37.6 $\pm$ 1.6 & 81.8 & 82.6 $\pm$ 1.4  & 52.6 & 58.9 $\pm$ 2.4 
% % & 71.2  & 78.1 $\pm$ 0.2 
% & 67.6 & 71.9 $\pm$ 1.0 & 77.0 & 79.7 $\pm$ 1.2\\
% \bottomrule
% \end{tabular}
% }
% \caption{The average performance (\%) of the involved 11 models (zero-shot) on the original and mimicked MMLU.  
% The update is conducted four times, and the table shows the average performance and the standard deviation.
% }
% \label{tab: mimic result mmlu}
% \vspace{-3mm}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It is apparent that: \textbf{1)} Compared with the performance of baselines on original datasets, their performance on our curated datasets are similar --- the difference of the two scores is 5\% on average except Element (we will discuss it later)
, 18\% max and 0\% min. 
This is mainly because the mimicked dataset has a similar style and difficulty; \textbf{2)} Among four different mimicked datasets, the standard deviation is limited, ranging from 0\% to 3\%. This demonstrates the stability of our mimicking dataset update strategy; \textbf{3)} The performance on the ``Periodic Elements'' in the mimicked dataset is markedly lower than in the original. This discrepancy can be attributed to the inclusion of the periodic table in the task description to assist the model in generating new questions. Unlike the original task, which exhaustively covered all possible one-hop questions like \textit{``What element contains one more proton than hydrogen?''}, the model, with the aid of the periodic table, generated more complex queries such as \textit{``What element contains two more protons than hydrogen?''}, which may need a reasoning step to answer compared to the original sample.
This also demonstrates the possibility of introducing external knowledge for updates, which will be future work.
\vspace{-2mm}
\subsection{Can mimicked datasets alleviate overestimation when data leakage occurs?}\label{Sec: how data leakage affect}
One of our main motivations is to automate dataset updates, so as to mitigate the overestimation caused by data leakage issues --- the pre-training procedure includes testing data, highlighted by~\cite{zhou2023don}. To simulate the data leakage issue, we finetune models using the testing data from original datasets (combined into one testing set) and evaluate them on our updated dataset to see if the performance is affected similarly or not. 
% We exclusively utilize a supervised fine-tuning (SFT) training setting, as data leakage during a model's pretraining phase can typically be detected by current contamination detection methods~\cite{shi2023detecting}. In contrast, our experiment demonstrates that when data leakage happened occurring during the SFT stage can not be effectively detected by cureent methods (detailed results of this investigation are provided in Appendix~\ref{appendix: Contamination Detection for the Finetuned Models}).  
 To simulate the data leakage issue, we choose four baseline models, Llama-2-7b-chat, Llama-2-13b-chat~\cite{llama2}, Llama-3-8b-Instruction~\cite{llama3} and Mistral-7b-instruction~\cite{mistral-7b}, and follow the training configuration in previous work~\cite{zhou2023don, llama2, xu2023wizardlm} for fair evaluation (detailed configuration is in the Appendix~\ref{model setting appendix}). For each model, there are three training settings: \textbf{1)} \textit{None}, which denotes the original model; \textbf{2)} \textit{leakage}, referring to the finetuned model using the above leakage simulation; \textbf{3)} \textit{w rationale}, which included rationales for each leakage sample during finetuning. Thus, these rationale finetuning will also improve the model's reasoning ability over the testing samples. In specific, we follow~\cite{wei2022finetuned} to generate rationales using GPT-4~\cite{GPT-4} for the correct choice. The detailed prompt is shown in the Appendix~\ref{ration creation}.
As shown in Table~\ref{tab: data leakge affect} and Table~\ref{tab: data leakge affect mmlu}, we find that: \textbf{1)} on the original dataset, the performance of all leakage simulations increases dramatically, no matter finetune via LoRA~\cite{hu2021lora} or not. This is consistent with previous works~\cite{zhou2023don}, showing the serious overestimation issue; \textbf{2)} on our mimicked datasets, the performance of all leakage simulations generally decreases or remains similar, except task Algos, and Algebra (will be discussed with the extending strategy); \textbf{3)} in most cases, the performance of \textit{leakage} setting is better than that of \textit{w rationale} on original datasets, while the results are opposite in mimicked datasets. We attribute this to the improvement of the generalization ability through training with rationales, which will depress/mitigate the overfitting performance of \textit{leakage}/\textit{w rationale}, aligned with~\cite{longpre2023flan}. 
\textbf{4)} Llama-2-13b gets improved from 3.4\% to 43.3\% on the task Algos after finetuning. We hypothesize this enhancement is attributable to model learning the distribution of labels, considering that the labels range uniformly from 1 to 10. This indicates a limitation of the mimicking strategy: the possibility of data leakage leading to models learning from the answer distribution, which in turn leads to an overestimated result.
% \begin{table*}[htb]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccc|cc|cc|cc|cc}
% \toprule
% \textbf{Model} &\textbf{Training} &\textbf{LoRa Only} &\textbf{Sports$_o$} &\textbf{Sports$_m$}& \textbf{Element$_o$} &\textbf{Element$_m$}& \textbf{Algos$_o$} 
% &\textbf{Algos$_m$}
% % & \textbf{conflict$_o$} &\textbf{conflict$_m$}
% & \textbf{Phys$_o$} &\textbf{Phys$_m$}& \textbf{Math$_o$} &\textbf{Math$_m$}\\

% \midrule
% Llama-7b & None & - &94.3 & 94.2 & 19.9 & 3.1 & 2.0 & 2.6
% % & 63.6 & 70.2 $\pm$ 0.4 
% & 44.4 & 57.5  & 14.6 & 15.1 \\
% Llama-7b & + leakage & \checkmark  & 99.7 & 87.4 & 57.1 & 0.9 & 42.2 & 34.0 & 74.9 & 51.3 & 43.6 & 18.0\\
% Llama-7b & + w rationale & \checkmark  & 92.4 & 92.7  & 39.9 & 1.3 & 37.2 & 36.0 & 67.9 & 57.5& 25.8 & 19.8\\
% Llama-7b &  + leakage & \ding{55} & 99.8 & 85.8 & 42.9 & 0.0 &32.5 & 25.3 & 70.4 & 52.5 & 42.0 & 19.2\\
% Llama-7b &  + w rationale & \ding{55} & 99.7 & 88.7 & 47.8 & 0.2 & 40.6 & 34.0 & 70.4 & 55.6 & 32.4 & 20.8\\
% \midrule
% Llama-13b & None & - & 92.7 & 96.1 & 27.8 & 4.0 & 6.1 & 3.4  
% % & 62.0 & 68.1
% & 54.3 & 58.5 & 19.6 & 24.6  \\
% Llama-13b & + leakage & \checkmark & 99.8 & 89.2 &  65.7 & 1.1 & 54.4 & 42.7
% % & 98.9 & 94.5 
% & 83.9 & 61.3 & 43.6 & 23.1 \\
% Llama-13b&  + w rationale & \checkmark  & 96.5& 91.7 & 49.3 & 1.8 & 45.6 & 43.3
% % & \textbf{99.7} & \textbf{97.6} 
% & 74.0 & 55.0&32.0 & 28.6\\
% % LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
% Llama-13b& +leakage & \ding{55} & 99.7 &88.5 & 40.7 & 0.0 &36.3 &28.0 & 71.6 &  45.0 & 42.3 & 26.4 \\
% Llama-13b& + w rationale & \ding{55} & 94.3 & 88.9 & 43.6 & 0.9 & 37.3 & 39.4 & 76.6 & 62.5 & 36.4 & 28.2\\
% \midrule
% Llama-8b& None & - & 98.2& 99.7 & 36.9 & 3.3& 4.1 & 6.0 & 70.4&67.5 & 43.9 & 34.8\\
% Llama-8b& +leakage &\checkmark & 98.7 & 92.5  &66.2 & 2.6  &36.6 & 39.3 & 77.8& 67.5 & 57.1 & 34.4\\
% Llama-8b& + w rationale &\checkmark & 98.1 & 87.7 & 68.2 & 7.5 & 39.4 & 44.0 & 86.9 & 71.3 &51.5 & 37.1\\
% Llama-8b& + w rationale &\ding{55} & 93.2 &85.6& 60.8& 12.4 & 36.6 & 39.3& 79.0 &66.3 &44.5 & 29.9\\
% \midrule
% Mistral-7b & None & - & 88.8 & 94.0 & 27.1 & 5.3 & 15.7 & 20.0
% % & 80.1 & 83.2 $\pm$ 0.6 
% &53.1 & 57.5  & 12.5 &25.8 \\
% Mistral-7b & + leakage & \checkmark & 99.8 & 87.7 & 36.6 & 1.6 &38.1 & 30.7 & 66.7 & 58.8 & 49.9 & 24.1\\
% Mistral-7b &  + w rationale & \checkmark & 95.0 & 90.4 & 54.8 & 1.6 & 46.6 & 40.6 & 81.0 & 58.8 & 34.4 & 21.5\\
% % Mistral-7b& + Test P \& S & \ding{55} & 61 &\\
% Mistral-7b&  + w rationale& \ding{55} & 98.3 & 88.2 & 61.0 & 0.0 & 45.9 & 38.0 & 88.9 & 56.8 & 48.0 & 27.5\\
% \bottomrule
% \end{tabular}}
% \caption{Finetune performance (\%) (zero-shot) of Llama-2-7b-chat, Llama-2-13b-chat and Mistral-7b-instruction on the original and mimicked BIG-bench examples (here we use the dataset from one of the iterations for time and cost consideration), \textit{leakage} denote use test prompt and the test set during training. \textit{w rationale} denote using test set with rational (detail in Sec~\ref{Sec: how data leakage affect}). For our fine-tuning process, we specifically employed: full parameter and Lora-only }
% \label{tab: data leakge affect}
% \end{table*}
 
 
 
 
 
%  \begin{table*}[htb]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccc|cc|cc|cc|cc}
% \toprule
% \textbf{Model} &\textbf{Training} &\textbf{LoRa Only} &\textbf{Sports$_o$} &\textbf{Sports$_m$}& \textbf{Element$_o$} &\textbf{Element$_m$}& \textbf{Algos$_o$} 
% &\textbf{Algos$_m$}
% % & \textbf{conflict$_o$} &\textbf{conflict$_m$}
% & \textbf{Phys$_o$} &\textbf{Phys$_m$}& \textbf{Math$_o$} &\textbf{Math$_m$}\\
% \midrule
% Llama-7b & None & - &94.3 & 94.2 & 19.9 & 3.1 & 2.0 & 2.6
% % & 63.6 & 70.2 $\pm$ 0.4 
% & 44.4 & 57.5  & 14.6 & 15.1 \\
% Llama-7b & + leakage & \checkmark  & 99.7 \textcolor{red}{(+5.4)} & 87.4 \textcolor{green}{(-6.8)} & 57.1 \textcolor{red}{(+37.2)} & 0.9 \textcolor{green}{(-2.2)} & 42.2 \textcolor{red}{(+40.2)} & 34.0 \textcolor{red}{(+31.4)} & 74.9 \textcolor{red}{(+30.5)} & 51.3 \textcolor{green}{(-6.2)} & 43.6 \textcolor{red}{(+29.0)} & 18.0 \textcolor{green}{(+2.9)}\\
% Llama-7b & + w rationale & \checkmark  & 92.4 \textcolor{green}{(-1.9)} & 92.7 \textcolor{green}{(-1.5)}  & 39.9 \textcolor{red}{(+20.0)} & 1.3 \textcolor{green}{(-1.8)} & 37.2 \textcolor{red}{(+35.2)} & 36.0 \textcolor{red}{(+33.4)} & 67.9 \textcolor{red}{(+23.5)} & 57.5 \textcolor{green}{(+0.0)}& 25.8 \textcolor{red}{(+11.2)} & 19.8 \textcolor{green}{(+4.7)}\\
% Llama-7b &  + leakage & \ding{55} & 99.8 \textcolor{red}{(+5.5)} & 85.8 \textcolor{green}{(-8.4)} & 42.9 \textcolor{red}{(+23.0)} & 0.0 \textcolor{green}{(-3.1)} &32.5 \textcolor{red}{(+30.5)} & 25.3 \textcolor{red}{(+22.7)} & 70.4 \textcolor{red}{(+26.0)} & 52.5 \textcolor{green}{(-5.0)} & 42.0 \textcolor{red}{(+27.4)} & 19.2 \textcolor{green}{(+4.1)}\\
% Llama-7b &  + w rationale & \ding{55} & 99.7 \textcolor{red}{(+5.4)} & 88.7 \textcolor{green}{(-5.5)} & 47.8 \textcolor{red}{(+27.9)} & 0.2 \textcolor{green}{(-2.9)} & 40.6 \textcolor{red}{(+38.6)} & 34.0 \textcolor{red}{(+31.4)} & 70.4 \textcolor{red}{(+26.0)} & 55.6 \textcolor{green}{(-1.9)} & 32.4 \textcolor{red}{(+17.8)} & 20.8 \textcolor{red}{(+5.7)} \\
% \midrule
% Llama-13b & None & - & 92.7 & 96.1 & 27.8 & 4.0 & 6.1 & 3.4  
% % & 62.0 & 68.1
% & 54.3 & 58.5 & 19.6 & 24.6  \\
% Llama-13b & + leakage & \checkmark & 99.8 \textcolor{red}{(+7.1)} & 89.2 \textcolor{green}{(-6.9)} &  65.7 \textcolor{red}{(+37.9)} & 1.1 \textcolor{green}{(-2.9)} & 54.4 \textcolor{red}{(+48.3)} & 42.7 \textcolor{red}{(+39.3)}
% % & 98.9 & 94.5 
% & 83.9 \textcolor{red}{(+29.6)} & 61.3 \textcolor{green}{(+2.8)} & 43.6 \textcolor{red}{(+24.0)} & 23.1 \textcolor{green}{(-1.5)} \\
% Llama-13b&  + w rationale & \checkmark  & 96.5 \textcolor{green}{(+3.8)}& 91.7 \textcolor{green}{(-4.4)} & 49.3 \textcolor{red}{(+21.5)} & 1.8 \textcolor{green}{(-2.2)} & 45.6 \textcolor{red}{(+39.5)} & 43.3 \textcolor{red}{(+39.9)}
% % & \textbf{99.7} & \textbf{97.6} 
% & 74.0 \textcolor{red}{(+19.7)}& 55.0 \textcolor{green}{(-3.5)}& 32.0 \textcolor{red}{(+12.4)} & 28.6 \textcolor{green}{(+4.0)}\\
% % LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
% Llama-13b& +leakage & \ding{55} & 99.7 \textcolor{red}{(+7.0)} &88.5 \textcolor{green}{(-7.6)} & 40.7 \textcolor{red}{(+12.9)} & 0.0 \textcolor{green}{(-4.0)} & 36.3 \textcolor{red}{(+30.2)} & 28.0 \textcolor{red}{(+24.6)} & 71.6 \textcolor{red}{(+17.3)} &  45.0 \textcolor{green}{(-13.5)} & 42.3 \textcolor{red}{(+22.7)} & 26.4 \textcolor{green}{(+1.8)} \\
% Llama-13b& + w rationale & \ding{55} & 94.3 \textcolor{green}{(+1.6)} & 88.9 \textcolor{green}{(-7.2)} & 43.6 \textcolor{red}{(+15.8)} & 0.9 \textcolor{green}{(-3.1)} & 37.3 \textcolor{red}{(+31.2)} & 39.4 \textcolor{red}{(+36.0)} & 76.6 \textcolor{red}{(+22.3)} & 62.5 \textcolor{green}{(+4.0)} & 36.4 \textcolor{red}{(+16.8)} & 28.2 \textcolor{green}{(+3.6)}\\
% \midrule
% Llama-8b & None & - & 98.2 & 99.7 & 36.9 & 3.3 & 4.1 & 6.0 & 70.4 & 67.5 & 43.9 & 34.8 \\
% Llama-8b & + leakage & \checkmark & 98.7 (\textcolor{green}{+0.5}) & 92.5 (\textcolor{green}{-7.2}) & 66.2 (\textcolor{red}{+29.3}) & 2.6 (\textcolor{green}{-0.7}) & 36.6 (\textcolor{red}{+32.5}) & 39.3 (\textcolor{red}{+33.3}) & 77.8 (\textcolor{red}{+7.4}) & 67.5 (\textcolor{green}{+0.0}) & 57.1 (\textcolor{red}{+13.2}) & 34.4 (\textcolor{green}{-0.4}) \\
% Llama-8b & + w rationale & \checkmark & 98.1 (\textcolor{green}{-0.1}) & 87.7 (\textcolor{green}{-12.0}) & 68.2 (\textcolor{red}{+31.3}) & 7.5 (\textcolor{green}{+4.2}) & 39.4 (\textcolor{red}{+35.3}) & 44.0 (\textcolor{red}{+38.0}) & 86.9 (\textcolor{red}{+16.5}) & 71.3 (\textcolor{green}{+3.8}) & 51.5 (\textcolor{red}{+7.6}) & 37.1 (\textcolor{green}{+2.3}) \\
% Llama-8b & + w rationale & \ding{55} & 93.2 (\textcolor{green}{-5.0}) & 85.6 (\textcolor{green}{-14.1}) & 60.8 (\textcolor{red}{+23.9}) & 12.4 (\textcolor{red}{+9.1}) & 36.6 (\textcolor{red}{+32.5}) & 39.3 (\textcolor{red}{+33.3}) & 79.0 (\textcolor{red}{+8.6}) & 66.3 (\textcolor{green}{-1.2}) & 44.5 (\textcolor{green}{+0.6}) & 29.9 (\textcolor{green}{-4.9}) \\
% \midrule
% Mistral-7b & None & - &88.8 & 94.0 & 27.1 & 5.3 & 15.7 & 20.0 & 53.1 & 57.5 & 12.5 & 25.8 \\
% Mistral-7b & + leakage & \checkmark & 99.8(\textcolor{red}{+11.0}) & 87.7(\textcolor{green}{-6.3}) & 36.6(\textcolor{red}{+9.5}) & 1.6(\textcolor{green}{-3.7}) & 38.1(\textcolor{red}{+22.4}) & 30.7(\textcolor{red}{+10.7}) & 66.7(\textcolor{red}{+13.6}) & 58.8(\textcolor{green}{+1.3}) & 49.9(\textcolor{red}{+37.4}) & 24.1(\textcolor{green}{-1.7}) \\
% Mistral-7b & + w rationale & \checkmark & 95.0(\textcolor{red}{+6.2}) & 90.4(\textcolor{green}{-3.6}) & 54.8(\textcolor{red}{+27.7}) & 1.6(\textcolor{green}{-3.7}) & 46.6(\textcolor{red}{+30.9}) & 40.6(\textcolor{red}{+20.6}) & 81.0(\textcolor{red}{+27.9}) & 58.8(\textcolor{green}{+1.3}) & 34.4(\textcolor{red}{+21.9}) & 21.5(\textcolor{green}{-4.3}) \\
% Mistral-7b & + w rationale & \ding{55} & 98.3(\textcolor{red}{+9.5}) & 88.2(\textcolor{green}{-5.8}) & 61.0(\textcolor{red}{+33.9}) & 0.0(\textcolor{green}{-5.3}) & 45.9(\textcolor{red}{+30.2}) & 38.0(\textcolor{red}{+18.0}) & 88.9(\textcolor{red}{+35.8}) & 56.8(\textcolor{green}{-0.7}) & 48.0(\textcolor{red}{+35.5}) & 27.5(\textcolor{green}{+1.7}) \\

% \bottomrule
% \end{tabular}}
% \caption{Finetune performance (\%) (zero-shot) of Llama-2-7b-chat, Llama-2-13b-chat and Mistral-7b-instruction on the original and mimicked BIG-bench examples (here we use the dataset from one of the iterations for time and cost consideration), \textit{leakage} denote use test prompt and the test set during training. \textit{w rationale} denote using test set with rational (detail in Sec~\ref{Sec: how data leakage affect}). For our fine-tuning process, we specifically employed: full parameter and Lora-only }
% \label{tab: data leakge affect}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
% \begin{table*}[htb]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccc|cc|cc|cc|cc}
% \toprule
% \textbf{Model} &\textbf{Training} &\textbf{LoRa Only} &\textbf{Sports$_o$} &\textbf{Sports$_m$}& \textbf{Element$_o$} &\textbf{Element$_m$}& \textbf{Algos$_o$} 
% &\textbf{Algos$_m$}
% % & \textbf{conflict$_o$} &\textbf{conflict$_m$}
% & \textbf{Phys$_o$} &\textbf{Phys$_m$}& \textbf{Math$_o$} &\textbf{Math$_m$}\\
% \midrule
% Llama-7b & None & - &94.3 & 94.2 & 19.9 & 3.1 & 2.0 & 2.6
% % & 63.6 & 70.2 $\pm$ 0.4 
% & 44.4 & 57.5  & 14.6 & 15.1 \\
% Llama-7b & + leakage & \checkmark  & 99.7 \textcolor{red}{(+5.4)} & 87.4 \textcolor{green}{(-6.8)} & 57.1 \textcolor{red}{(+37.2)} & 0.9 \textcolor{green}{(-2.2)} & 42.2 \textcolor{red}{(+40.2)} & 34.0 \textcolor{red}{(+31.4)} & 74.9 \textcolor{red}{(+30.5)} & 51.3 \textcolor{green}{(-6.2)} & 43.6 \textcolor{red}{(+29.0)} & 18.0 \textcolor{green}{(+2.9)}\\
% Llama-7b & + w rationale & \checkmark  & 92.4 \textcolor{green}{(-1.9)} & 92.7 \textcolor{green}{(-1.5)}  & 39.9 \textcolor{red}{(+20.0)} & 1.3 \textcolor{green}{(-1.8)} & 37.2 \textcolor{red}{(+35.2)} & 36.0 \textcolor{red}{(+33.4)} & 67.9 \textcolor{red}{(+23.5)} & 57.5 \textcolor{green}{(+0.0)}& 25.8 \textcolor{red}{(+11.2)} & 19.8 \textcolor{green}{(+4.7)}\\
% Llama-7b &  + leakage & \ding{55} & 99.8 \textcolor{red}{(+5.5)} & 85.8 \textcolor{green}{(-8.4)} & 42.9 \textcolor{red}{(+23.0)} & 0.0 \textcolor{green}{(-3.1)} &32.5 \textcolor{red}{(+30.5)} & 25.3 \textcolor{red}{(+22.7)} & 70.4 \textcolor{red}{(+26.0)} & 52.5 \textcolor{green}{(-5.0)} & 42.0 \textcolor{red}{(+27.4)} & 19.2 \textcolor{green}{(+4.1)}\\
% Llama-7b &  + w rationale & \ding{55} & 99.7 \textcolor{red}{(+5.4)} & 88.7 \textcolor{green}{(-5.5)} & 47.8 \textcolor{red}{(+27.9)} & 0.2 \textcolor{green}{(-2.9)} & 40.6 \textcolor{red}{(+38.6)} & 34.0 \textcolor{red}{(+31.4)} & 70.4 \textcolor{red}{(+26.0)} & 55.6 \textcolor{green}{(-1.9)} & 32.4 \textcolor{red}{(+17.8)} & 20.8 \textcolor{red}{(+5.7)} \\
% \midrule
% Llama-13b & None & - & 92.7 & 96.1 & 27.8 & 4.0 & 6.1 & 3.4  
% % & 62.0 & 68.1
% & 54.3 & 58.5 & 19.6 & 24.6  \\
% Llama-13b & + leakage & \checkmark & 99.8 \textcolor{red}{(+7.1)} & 89.2 \textcolor{green}{(-6.9)} &  65.7 \textcolor{red}{(+37.9)} & 1.1 \textcolor{green}{(-2.9)} & 54.4 \textcolor{red}{(+48.3)} & 42.7 \textcolor{red}{(+39.3)}
% % & 98.9 & 94.5 
% & 83.9 \textcolor{red}{(+29.6)} & 61.3 \textcolor{green}{(+2.8)} & 43.6 \textcolor{red}{(+24.0)} & 23.1 \textcolor{green}{(-1.5)} \\
% Llama-13b&  + w rationale & \checkmark  & 96.5 \textcolor{green}{(+3.8)}& 91.7 \textcolor{green}{(-4.4)} & 49.3 \textcolor{red}{(+21.5)} & 1.8 \textcolor{green}{(-2.2)} & 45.6 \textcolor{red}{(+39.5)} & 43.3 \textcolor{red}{(+39.9)}
% % & \textbf{99.7} & \textbf{97.6} 
% & 74.0 \textcolor{red}{(+19.7)}& 55.0 \textcolor{green}{(-3.5)}& 32.0 \textcolor{red}{(+12.4)} & 28.6 \textcolor{green}{(+4.0)}\\
% % LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
% Llama-13b& +leakage & \ding{55} & 99.7 \textcolor{red}{(+7.0)} &88.5 \textcolor{green}{(-7.6)} & 40.7 \textcolor{red}{(+12.9)} & 0.0 \textcolor{green}{(-4.0)} & 36.3 \textcolor{red}{(+30.2)} & 28.0 \textcolor{red}{(+24.6)} & 71.6 \textcolor{red}{(+17.3)} &  45.0 \textcolor{green}{(-13.5)} & 42.3 \textcolor{red}{(+22.7)} & 26.4 \textcolor{green}{(+1.8)} \\
% Llama-13b& + w rationale & \ding{55} & 94.3 \textcolor{green}{(+1.6)} & 88.9 \textcolor{green}{(-7.2)} & 43.6 \textcolor{red}{(+15.8)} & 0.9 \textcolor{green}{(-3.1)} & 37.3 \textcolor{red}{(+31.2)} & 39.4 \textcolor{red}{(+36.0)} & 76.6 \textcolor{red}{(+22.3)} & 62.5 \textcolor{green}{(+4.0)} & 36.4 \textcolor{red}{(+16.8)} & 28.2 \textcolor{green}{(+3.6)}\\
% \midrule
% Llama-8b & None & - & 98.2 & 99.7 & 36.9 & 3.3 & 4.1 & 6.0 & 70.4 & 67.5 & 43.9 & 34.8 \\
% Llama-8b & + leakage & \checkmark & 98.7 (\textcolor{green}{+0.5}) & 92.5 (\textcolor{green}{-7.2}) & 66.2 (\textcolor{red}{+29.3}) & 2.6 (\textcolor{green}{-0.7}) & 36.6 (\textcolor{red}{+32.5}) & 39.3 (\textcolor{red}{+33.3}) & 77.8 (\textcolor{red}{+7.4}) & 67.5 (\textcolor{green}{+0.0}) & 57.1 (\textcolor{red}{+13.2}) & 34.4 (\textcolor{green}{-0.4}) \\
% Llama-8b & + w rationale & \checkmark & 98.1 (\textcolor{green}{-0.1}) & 87.7 (\textcolor{green}{-12.0}) & 68.2 (\textcolor{red}{+31.3}) & 7.5 (\textcolor{green}{+4.2}) & 39.4 (\textcolor{red}{+35.3}) & 44.0 (\textcolor{red}{+38.0}) & 86.9 (\textcolor{red}{+16.5}) & 71.3 (\textcolor{green}{+3.8}) & 51.5 (\textcolor{red}{+7.6}) & 37.1 (\textcolor{green}{+2.3}) \\
% Llama-8b & + w rationale & \ding{55} & 93.2 (\textcolor{green}{-5.0}) & 85.6 (\textcolor{green}{-14.1}) & 60.8 (\textcolor{red}{+23.9}) & 12.4 (\textcolor{red}{+9.1}) & 36.6 (\textcolor{red}{+32.5}) & 39.3 (\textcolor{red}{+33.3}) & 79.0 (\textcolor{red}{+8.6}) & 66.3 (\textcolor{green}{-1.2}) & 44.5 (\textcolor{green}{+0.6}) & 29.9 (\textcolor{green}{-4.9}) \\
% \midrule
% Mistral-7b & None & - &88.8 & 94.0 & 27.1 & 5.3 & 15.7 & 20.0 & 53.1 & 57.5 & 12.5 & 25.8 \\
% Mistral-7b & + leakage & \checkmark & 99.8(\textcolor{red}{+11.0}) & 87.7(\textcolor{green}{-6.3}) & 36.6(\textcolor{red}{+9.5}) & 1.6(\textcolor{green}{-3.7}) & 38.1(\textcolor{red}{+22.4}) & 30.7(\textcolor{red}{+10.7}) & 66.7(\textcolor{red}{+13.6}) & 58.8(\textcolor{green}{+1.3}) & 49.9(\textcolor{red}{+37.4}) & 24.1(\textcolor{green}{-1.7}) \\
% Mistral-7b & + w rationale & \checkmark & 95.0(\textcolor{red}{+6.2}) & 90.4(\textcolor{green}{-3.6}) & 54.8(\textcolor{red}{+27.7}) & 1.6(\textcolor{green}{-3.7}) & 46.6(\textcolor{red}{+30.9}) & 40.6(\textcolor{red}{+20.6}) & 81.0(\textcolor{red}{+27.9}) & 58.8(\textcolor{green}{+1.3}) & 34.4(\textcolor{red}{+21.9}) & 21.5(\textcolor{green}{-4.3}) \\
% Mistral-7b & + w rationale & \ding{55} & 98.3(\textcolor{red}{+9.5}) & 88.2(\textcolor{green}{-5.8}) & 61.0(\textcolor{red}{+33.9}) & 0.0(\textcolor{green}{-5.3}) & 45.9(\textcolor{red}{+30.2}) & 38.0(\textcolor{red}{+18.0}) & 88.9(\textcolor{red}{+35.8}) & 56.8(\textcolor{green}{-0.7}) & 48.0(\textcolor{red}{+35.5}) & 27.5(\textcolor{green}{+1.7}) \\

% \bottomrule
% \end{tabular}}
% \caption{Finetune performance (\%) (zero-shot) of Llama-2-7b-chat, Llama-2-13b-chat and Mistral-7b-instruction on the original and mimicked BIG-bench examples (here we use the dataset from one of the iterations for time and cost consideration), \textit{leakage} denote use test prompt and the test set during training. \textit{w rationale} denote using test set with rational (detail in Sec~\ref{Sec: how data leakage affect}). For our fine-tuning process, we specifically employed: full parameter and Lora-only }
% \label{tab: data leakge affect}
% \end{table*}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \begin{table*}[htb]
 \vspace{-3mm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc|cc|cc|cc|cc}
\toprule
\textbf{Model} &\textbf{Training} &\textbf{LoRA Only} &\textbf{Sports$_o$} &\textbf{Sports$_m$}& \textbf{Element$_o$} &\textbf{Element$_m$}& \textbf{Algos$_o$} 
&\textbf{Algos$_m$}
% & \textbf{conflict$_o$} &\textbf{conflict$_m$}
& \textbf{Phys$_o$} &\textbf{Phys$_m$}& \textbf{Math$_o$} &\textbf{Math$_m$}\\
\midrule
Llama-7b & None & - &94.3 & 94.2 & 19.9 & 3.1 & 2.0 & 2.6
% & 63.6 & 70.2 $\pm$ 0.4 
& 44.4 & 57.5  & 14.6 & 15.1 \\
% Llama-7b & + leakage & \checkmark  & 99.7 \textcolor{red}{(+5.4)} & 87.4 \textcolor{green}{(-6.8)} & 57.1 \textcolor{red}{(+37.2)} & 0.9 \textcolor{green}{(-2.2)} & 42.2 \textcolor{red}{(+40.2)} & 34.0 \textcolor{red}{(+31.4)} & 74.9 \textcolor{red}{(+30.5)} & 51.3 \textcolor{green}{(-6.2)} & 43.6 \textcolor{red}{(+29.0)} & 18.0 \textcolor{green}{(+2.9)}\\
% Llama-7b & + w rationale & \checkmark  & 92.4 \textcolor{green}{(-1.9)} & 92.7 \textcolor{green}{(-1.5)}  & 39.9 \textcolor{red}{(+20.0)} & 1.3 \textcolor{green}{(-1.8)} & 37.2 \textcolor{red}{(+35.2)} & 36.0 \textcolor{red}{(+33.4)} & 67.9 \textcolor{red}{(+23.5)} & 57.5 \textcolor{green}{(+0.0)}& 25.8 \textcolor{red}{(+11.2)} & 19.8 \textcolor{green}{(+4.7)}\\
% Llama-7b &  + leakage & \ding{55} & 99.8 \textcolor{red}{(+5.5)} & 85.8 \textcolor{green}{(-8.4)} & 42.9 \textcolor{red}{(+23.0)} & 0.0 \textcolor{green}{(-3.1)} &32.5 \textcolor{red}{(+30.5)} & 25.3 \textcolor{red}{(+22.7)} & 70.4 \textcolor{red}{(+26.0)} & 52.5 \textcolor{green}{(-5.0)} & 42.0 \textcolor{red}{(+27.4)} & 19.2 \textcolor{green}{(+4.1)}\\
% Llama-7b &  + w rationale & \ding{55} & 99.7 \textcolor{red}{(+5.4)} & 88.7 \textcolor{green}{(-5.5)} & 47.8 \textcolor{red}{(+27.9)} & 0.2 \textcolor{green}{(-2.9)} & 40.6 \textcolor{red}{(+38.6)} & 34.0 \textcolor{red}{(+31.4)} & 70.4 \textcolor{red}{(+26.0)} & 55.6 \textcolor{green}{(-1.9)} & 32.4 \textcolor{red}{(+17.8)} & 20.8 \textcolor{red}{(+5.7)} \\
% \midrule
% Llama-7b & + leakage & \checkmark & 99.7 (3) & 87.4 (5) & 57.1 (1) & 0.9 (5) & 42.2 (1) & 34.0 (1) & 74.9 (1) & 51.3 (5) & 43.6 (2) & 18.0 (4) \\
% Llama-7b & + w rationale & \checkmark & 92.4 (5) & 92.7 (5) & 39.9 (2) & 1.3 (5) & 37.2 (1) & 36.0 (1) & 67.9 (2) & 57.5 (4) & 25.8 (2) & 19.8 (4) \\
% Llama-7b & + leakage & \ding{55} & 99.8 (3) & 85.8 (5) & 42.9 (2) & 0.0 (5) & 32.5 (1) & 25.3 (2) & 70.4 (2) & 52.5 (5) & 42.0 (2) & 19.2 (4) \\
% Llama-7b & + w rationale & \ding{55} & 99.7 (3) & 88.7 (5) & 47.8 (2) & 0.2 (5) & 40.6 (1) & 34.0 (1) & 70.4 (2) & 55.6 (5) & 32.4 (2) & 20.8 (3) \\
% \midrule
Llama2-7b & + leakage & \checkmark & \cellcolor{extremelylightred} 99.7 & \cellcolor{medblue} 87.4 & \cellcolor{lightred} 57.1 & \cellcolor{medblue} 0.9 & \cellcolor{lightred} 42.2 & \cellcolor{lightred} 34.0 & \cellcolor{lightred} 74.9 & \cellcolor{medblue} 51.3 & \cellcolor{verylightred} 43.6 & \cellcolor{lightblue} 18.0 \\
Llama2-7b & + w rationale & \checkmark & \cellcolor{medblue} 92.4 & \cellcolor{medblue} 92.7 & \cellcolor{verylightred} 39.9 & \cellcolor{medblue} 1.3 & \cellcolor{lightred} 37.2 & \cellcolor{lightred} 36.0 & \cellcolor{verylightred} 67.9 & \cellcolor{lightblue} 57.5 & \cellcolor{verylightred} 25.8 & \cellcolor{lightblue} 19.8 \\
Llama2-7b & + leakage & \ding{55} & \cellcolor{extremelylightred} 99.8 & \cellcolor{medblue} 85.8 & \cellcolor{verylightred} 42.9 & \cellcolor{medblue} 0.0 & \cellcolor{lightred} 32.5 & \cellcolor{verylightred} 25.3 & \cellcolor{verylightred} 70.4 & \cellcolor{medblue} 52.5 & \cellcolor{verylightred} 42.0 & \cellcolor{lightblue} 19.2 \\
Llama2-7b & + w rationale & \ding{55} & \cellcolor{extremelylightred} 99.7 & \cellcolor{medblue} 88.7 & \cellcolor{verylightred} 47.8 & \cellcolor{medblue} 0.2 & \cellcolor{lightred} 40.6 & \cellcolor{lightred} 34.0 & \cellcolor{verylightred} 70.4 & \cellcolor{medblue} 55.6 & \cellcolor{verylightred} 32.4 & \cellcolor{extremelylightred} 20.8 \\
\midrule
Llama2-13b & None & - & 92.7 & 96.1 & 27.8 & 4.0 & 6.1 & 3.4  
% & 62.0 & 68.1
& 54.3 & 58.5 & 19.6 & 24.6  \\
% Llama-13b & + leakage & \checkmark & 99.8 \textcolor{red}{(+7.1)} & 89.2 \textcolor{green}{(-6.9)} &  65.7 \textcolor{red}{(+37.9)} & 1.1 \textcolor{green}{(-2.9)} & 54.4 \textcolor{red}{(+48.3)} & 42.7 \textcolor{red}{(+39.3)}
% % & 98.9 & 94.5 
% & 83.9 \textcolor{red}{(+29.6)} & 61.3 \textcolor{green}{(+2.8)} & 43.6 \textcolor{red}{(+24.0)} & 23.1 \textcolor{green}{(-1.5)} \\
% Llama-13b&  + w rationale & \checkmark  & 96.5 \textcolor{green}{(+3.8)}& 91.7 \textcolor{green}{(-4.4)} & 49.3 \textcolor{red}{(+21.5)} & 1.8 \textcolor{green}{(-2.2)} & 45.6 \textcolor{red}{(+39.5)} & 43.3 \textcolor{red}{(+39.9)}
% % & \textbf{99.7} & \textbf{97.6} 
% & 74.0 \textcolor{red}{(+19.7)}& 55.0 \textcolor{green}{(-3.5)}& 32.0 \textcolor{red}{(+12.4)} & 28.6 \textcolor{green}{(+4.0)}\\
% % LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
% Llama-13b& +leakage & \ding{55} & 99.7 \textcolor{red}{(+7.0)} &88.5 \textcolor{green}{(-7.6)} & 40.7 \textcolor{red}{(+12.9)} & 0.0 \textcolor{green}{(-4.0)} & 36.3 \textcolor{red}{(+30.2)} & 28.0 \textcolor{red}{(+24.6)} & 71.6 \textcolor{red}{(+17.3)} &  45.0 \textcolor{green}{(-13.5)} & 42.3 \textcolor{red}{(+22.7)} & 26.4 \textcolor{green}{(+1.8)} \\
% Llama-13b& + w rationale & \ding{55} & 94.3 \textcolor{green}{(+1.6)} & 88.9 \textcolor{green}{(-7.2)} & 43.6 \textcolor{red}{(+15.8)} & 0.9 \textcolor{green}{(-3.1)} & 37.3 \textcolor{red}{(+31.2)} & 39.4 \textcolor{red}{(+36.0)} & 76.6 \textcolor{red}{(+22.3)} & 62.5 \textcolor{green}{(+4.0)} & 36.4 \textcolor{red}{(+16.8)} & 28.2 \textcolor{green}{(+3.6)}\\
% \midrule
% Llama-13b & + leakage & \checkmark & 99.8 (3) & 89.2 (5) &  65.7 (1) & 1.1 (5) & 54.4 (1) & 42.7 (1) & 83.9 (2) & 61.3 (4) & 43.6 (2) & 23.1 (5) \\
% Llama-13b&  + w rationale & \checkmark  & 96.5 (4) & 91.7 (5) & 49.3 (2) & 1.8 (5) & 45.6 (1) & 43.3 (1) & 74.0 (2) & 55.0 (5) & 32.0 (2) & 28.6 (4) \\
% Llama-13b& +leakage & \ding{55} & 99.7 (3) & 88.5 (5) & 40.7 (2) & 0.0 (5) & 36.3 (1) & 28.0 (2) & 71.6 (2) &  45.0 (5) & 42.3 (2) & 26.4 (4) \\
% Llama-13b& + w rationale & \ding{55} & 94.3 (4) & 88.9 (5) & 43.6 (2) & 0.9 (5) & 37.3 (1) & 39.4 (1) & 76.6 (2) & 62.5 (4) & 36.4 (2) & 28.2 (4) \\
% \midrule
Llama2-13b & + leakage & \checkmark & \cellcolor{extremelylightred} 99.8 & \cellcolor{medblue} 89.2 &  \cellcolor{lightred} 65.7 & \cellcolor{medblue} 1.1 & \cellcolor{lightred} 54.4 & \cellcolor{lightred} 42.7 & \cellcolor{verylightred} 83.9 & \cellcolor{lightblue} 61.3 & \cellcolor{verylightred} 43.6 & \cellcolor{medblue} 23.1 \\
Llama2-13b&  + w rationale & \checkmark  & \cellcolor{lightblue} 96.5 & \cellcolor{medblue} 91.7 & \cellcolor{verylightred} 49.3 & \cellcolor{medblue} 1.8 & \cellcolor{lightred} 45.6 & \cellcolor{lightred} 43.3 & \cellcolor{verylightred} 74.0 & \cellcolor{medblue} 55.0 & \cellcolor{verylightred} 32.0 & \cellcolor{lightblue} 28.6 \\
Llama2-13b& +leakage & \ding{55} & \cellcolor{extremelylightred} 99.7 & \cellcolor{medblue} 88.5 & \cellcolor{verylightred} 40.7 & \cellcolor{medblue} 0.0 & \cellcolor{lightred} 36.3 & \cellcolor{verylightred} 28.0 & \cellcolor{verylightred} 71.6 & \cellcolor{medblue} 45.0 & \cellcolor{verylightred} 42.3 & \cellcolor{lightblue} 26.4 \\
Llama2-13b& + w rationale & \ding{55} & \cellcolor{lightblue} 94.3 & \cellcolor{medblue} 88.9 & \cellcolor{verylightred} 43.6 & \cellcolor{medblue} 0.9 & \cellcolor{lightred} 37.3 & \cellcolor{lightred} 39.4 & \cellcolor{verylightred} 76.6 & \cellcolor{lightblue} 62.5 & \cellcolor{verylightred} 36.4 & \cellcolor{lightblue} 28.2 \\

\midrule
Llama2-8b & None & - & 98.2 & 99.7 & 36.9 & 3.3 & 4.1 & 6.0 & 70.4 & 67.5 & 43.9 & 34.8 \\
% Llama-8b & + leakage & \checkmark & 98.7 (\textcolor{green}{+0.5}) & 92.5 (\textcolor{green}{-7.2}) & 66.2 (\textcolor{red}{+29.3}) & 2.6 (\textcolor{green}{-0.7}) & 36.6 (\textcolor{red}{+32.5}) & 39.3 (\textcolor{red}{+33.3}) & 77.8 (\textcolor{red}{+7.4}) & 67.5 (\textcolor{green}{+0.0}) & 57.1 (\textcolor{red}{+13.2}) & 34.4 (\textcolor{green}{-0.4}) \\
% Llama-8b & + w rationale & \checkmark & 98.1 (\textcolor{green}{-0.1}) & 87.7 (\textcolor{green}{-12.0}) & 68.2 (\textcolor{red}{+31.3}) & 7.5 (\textcolor{green}{+4.2}) & 39.4 (\textcolor{red}{+35.3}) & 44.0 (\textcolor{red}{+38.0}) & 86.9 (\textcolor{red}{+16.5}) & 71.3 (\textcolor{green}{+3.8}) & 51.5 (\textcolor{red}{+7.6}) & 37.1 (\textcolor{green}{+2.3}) \\
% Llama-8b & + w rationale & \ding{55} & 93.2 (\textcolor{green}{-5.0}) & 85.6 (\textcolor{green}{-14.1}) & 60.8 (\textcolor{red}{+23.9}) & 12.4 (\textcolor{red}{+9.1}) & 36.6 (\textcolor{red}{+32.5}) & 39.3 (\textcolor{red}{+33.3}) & 79.0 (\textcolor{red}{+8.6}) & 66.3 (\textcolor{green}{-1.2}) & 44.5 (\textcolor{green}{+0.6}) & 29.9 (\textcolor{green}{-4.9}) \\
% \midrule
% Llama-8b & + leakage & \checkmark & 98.7 (4) & 92.5 (5) & 66.2 (2) & 2.6 (5) & 36.6 (1) & 39.3 (1) & 77.8 (3) & 67.5 (4) & 57.1 (2) & 34.4 (5) \\
% Llama-8b & + w rationale & \checkmark & 98.1 (5) & 87.7 (5) & 68.2 (1) & 7.5 (4) & 39.4 (1) & 44.0 (1) & 86.9 (2) & 71.3 (4) & 51.5 (3) & 37.1 (4) \\
% Llama-8b & + w rationale & \ding{55} & 93.2 (5) & 85.6 (5) & 60.8 (2) & 12.4 (3) & 36.6 (1) & 39.3 (1) & 79.0 (3) & 66.3 (5) & 44.5 (4) & 29.9 (5) \\
% \midrule
Llama3-8b & + leakage & \checkmark & \cellcolor{lightblue}98.7 & \cellcolor{medblue}92.5 & \cellcolor{verylightred}66.2 & \cellcolor{medblue}2.6 & \cellcolor{lightred}36.6 & \cellcolor{lightred}39.3 & \cellcolor{extremelylightred}77.8 & \cellcolor{lightblue}67.5 & \cellcolor{verylightred}57.1 & \cellcolor{medblue}34.4 \\
Llama3-8b & + w rationale & \checkmark & \cellcolor{medblue}98.1 & \cellcolor{medblue}87.7 & \cellcolor{lightred}68.2 & \cellcolor{lightblue}7.5 & \cellcolor{lightred}39.4 & \cellcolor{lightred}44.0 & \cellcolor{verylightred}86.9 & \cellcolor{lightblue}71.3 & \cellcolor{extremelylightred}51.5 & \cellcolor{lightblue}37.1 \\
Llama3-8b & + w rationale & \ding{55} & \cellcolor{medblue}93.2 & \cellcolor{medblue}85.6 & \cellcolor{verylightred}60.8 & \cellcolor{extremelylightred}12.4 & \cellcolor{lightred}36.6 & \cellcolor{lightred}39.3 & \cellcolor{extremelylightred}79.0 & \cellcolor{medblue}66.3 & \cellcolor{lightblue}44.5 & \cellcolor{medblue}29.9 \\
\midrule
Mistral-7b & None & - &88.8 & 94.0 & 27.1 & 5.3 & 15.7 & 20.0 & 53.1 & 57.5 & 12.5 & 25.8 \\
% Mistral-7b & + leakage & \checkmark & 99.8(\textcolor{red}{+11.0}) & 87.7(\textcolor{green}{-6.3}) & 36.6(\textcolor{red}{+9.5}) & 1.6(\textcolor{green}{-3.7}) & 38.1(\textcolor{red}{+22.4}) & 30.7(\textcolor{red}{+10.7}) & 66.7(\textcolor{red}{+13.6}) & 58.8(\textcolor{green}{+1.3}) & 49.9(\textcolor{red}{+37.4}) & 24.1(\textcolor{green}{-1.7}) \\
% Mistral-7b & + w rationale & \checkmark & 95.0(\textcolor{red}{+6.2}) & 90.4(\textcolor{green}{-3.6}) & 54.8(\textcolor{red}{+27.7}) & 1.6(\textcolor{green}{-3.7}) & 46.6(\textcolor{red}{+30.9}) & 40.6(\textcolor{red}{+20.6}) & 81.0(\textcolor{red}{+27.9}) & 58.8(\textcolor{green}{+1.3}) & 34.4(\textcolor{red}{+21.9}) & 21.5(\textcolor{green}{-4.3}) \\
% Mistral-7b & + w rationale & \ding{55} & 98.3(\textcolor{red}{+9.5}) & 88.2(\textcolor{green}{-5.8}) & 61.0(\textcolor{red}{+33.9}) & 0.0(\textcolor{green}{-5.3}) & 45.9(\textcolor{red}{+30.2}) & 38.0(\textcolor{red}{+18.0}) & 88.9(\textcolor{red}{+35.8}) & 56.8(\textcolor{green}{-0.7}) & 48.0(\textcolor{red}{+35.5}) & 27.5(\textcolor{green}{+1.7}) \\
% \midrule
% Mistral-7b & + leakage & \checkmark & 99.8 (2) & 87.7 (5) & 36.6 (3) & 1.6 (5) & 38.1 (2) & 30.7 (2) & 66.7 (2) & 58.8 (4) & 49.9 (1) & 24.1 (5) \\
% Mistral-7b & + w rationale & \checkmark & 95.0 (3) & 90.4 (5) & 54.8 (2) & 1.6 (5) & 46.6 (1) & 40.6 (2) & 81.0 (2) & 58.8 (4) & 34.4 (2) & 21.5 (5) \\
% Mistral-7b & + w rationale & \ding{55} & 98.3 (3) & 88.2 (5) & 61.0 (1) & 0.0 (5) & 45.9 (1) & 38.0 (2) & 88.9 (1) & 56.8 (5) & 48.0 (1) & 27.5 (4) \\
Mistral-7b & + leakage & \checkmark & \cellcolor{verylightred}99.8 & \cellcolor{medblue}87.7 & \cellcolor{extremelylightred}36.6 & \cellcolor{medblue}1.6 & \cellcolor{verylightred}38.1 & \cellcolor{verylightred}30.7 & \cellcolor{verylightred}66.7 & \cellcolor{lightblue}58.8 & \cellcolor{lightred}49.9 & \cellcolor{medblue}24.1 \\
Mistral-7b & + w rationale & \checkmark & \cellcolor{extremelylightred}95.0 & \cellcolor{medblue}90.4 & \cellcolor{verylightred}54.8 & \cellcolor{medblue}1.6 & \cellcolor{lightred}46.6 & \cellcolor{verylightred}40.6 & \cellcolor{verylightred}81.0 & \cellcolor{lightblue}58.8 & \cellcolor{verylightred}34.4 & \cellcolor{medblue}21.5 \\
Mistral-7b & + w rationale & \ding{55} & \cellcolor{extremelylightred}98.3 & \cellcolor{medblue}88.2 & \cellcolor{lightred}61.0 & \cellcolor{medblue}0.0 & \cellcolor{lightred}45.9 & \cellcolor{verylightred}38.0 & \cellcolor{lightred}88.9 & \cellcolor{medblue}56.8 & \cellcolor{lightred}48.0 & \cellcolor{lightblue}27.5 \\
\bottomrule
\end{tabular}}
\caption{Finetune performance (\%) (zero-shot) of Llama-2-7b-chat, Llama-2-13b-chat, Llama-3-8b-Instruction and Mistral-7b-instruction on the original and mimicked BIG-bench examples (here we use the dataset from one of the iterations for time and cost consideration), \textit{leakage} denote use test prompt and the test set during training. \textit{w rationale} denote using test set with rational (Sec~\ref{Sec: how data leakage affect}). For our fine-tuning process, we specifically employed: full parameter and LoRA-only. Cells are blue if finetuning boosts the performance less than 5\% else are in red. Specifically, \uniformbox{CBE1EE}{0.2cm}{less than 0\%},  \uniformbox{E4F0F7}{0.2cm}{mora than 0 \% but less than 5\%}, \uniformbox{FCF4EF}{0.2cm}{mora than 5 \% but less than 10\%}, \uniformbox{F5E1D9}{0.2cm}{more than 10 \%}.} 
\label{tab: data leakge affect}
\vspace{-1mm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 %
%  \begin{table*}[htb]
%  \vspace{-2mm}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccc|cc|cc|cc|cc}
% \toprule
% \textbf{Model} &\textbf{Training} & \textbf{LoRa Only}& \textbf{Algebra$_o$} &\textbf{Algebra$_m$}& \textbf{Law$_o$} &\textbf{Law$_m$}& \textbf{Econ$_o$} 
% &\textbf{Econ$_m$} & \textbf{Medicine$_o$} &\textbf{Medicine$_m$}& \textbf{Security$_o$} &\textbf{Security$_m$}\\
 
% \midrule
% Llama-7b & None & -&14.0 & 17.2  & 57.8 & 70.0  & 28.1 & 32.7
% % & 63.6 & 70.2 $\pm$ 0.4 
% & 41.9 & 49.8 & 58.0 & 60.0 \\
% Llama-7b & +leakage &\checkmark & 52.0 & 31.2 & 95.9 & 70.8 & 65.8 & 34.6 & 79.8 & 50.4 & 86.0 & 66.0\\
% Llama-7b & + w rationale & \checkmark &33.0 & 30.1 & 74.4 & 72.7 & 38.6&31.7 & 53.8 & 50.8 & 67.0 & 60.0\\
% Llama-7b &  + leakage &\ding{55} & 49.0 & 23.7 & 93.4 & 70.9 & 65.8 & 33.6 & 79.2 & 51.1 & 84.0 & 60.0\\
% Llama-7b&  + w rationale &  \ding{55} &  42.0 & 31.2 & 81.8 &73.5 & 46.5 & 36.6 & 62.4 & 55.0 & 76.0 & 63.0\\
% \midrule
% Llama-13b& None &-  & 31.0 & 29.0 & 70.0 & 77.8 & 30.0 & 36.7 
% % & 62.0 & 68.1 $\pm$ 0.8 
% &43.6  & 50.1  & 65.0 & 72.0  \\
% Llama-13b& + leakage & \checkmark & 51.0 & 30.1 & 96.7& 79.5 & 67.5 & 42.5 & 83.2 & 54.9 & 92.0 & 76.0 \\
% Llama-13b&  + w rationale & \checkmark & 34.0 & 32.6 & 86.0 & 80.5 & 39.5 & 40.2 & 58.4 & 55.5 & 75.0 & 74.0\\
% % LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
% Llama-13b& + leakage &  \ding{55} & 48.0 & 23.7 & 92.6 & 70.9 & 60.5 & 36.6 & 82.1 &50.4 &83.0 & 71.0\\
% Llama-13b&  + w rationale &  \ding{55} & 38.0 & 35.4 & 86.7 & 80.1 & 50.0 & 40.5 & 65.3 & 55.6& 79.0 &74.0\\
% \midrule
% Llama-8b& None & - & 34.0 & 36.5 & 76.9 & 82.0 & 50.9 & 59.4 & 65.9 & 70.3 & 74.0 & 81.0\\
% Llama-8b& + leakage & \checkmark & 49.0 & 29.0 & 92.6 & 83.7 & 72.8 &  61.3 & 87.2 & 75.0  & 89.0 & 80.0\\
% Llama-8b& + w rationale & \checkmark & 48.0 & 38.7 & 88.4 & 83.7 & 65.8 & 63.4 & 74.6 & 71.8 & 88.0 & 84.0\\ 
% % Llama-8b&  + leakage &  \ding{55} & 48.0 & 39.8 & 90.0 & 85.5 & 64.9 & 59.4 & 80.4 & 73.8 & 89.0 & 82.0\\
% Llama-8b&  + w rationale &  \ding{55} & 54.0 & 39.7 & 90.1 & 87.2 &74.6 & 61.3 & 76.3 &76.2 & 80.0 &83.0\\
% \midrule
% Mistral-7b & None & -& 34.0 & 26.8 & 70.2 & 77.1& 36.9 & 45.7  
% % & 80.1 & 83.2 $\pm$ 0.6 
% & 59.5 & 59.3  & 70.0 &  74.0\\
% Mistral-7b &  + leakage & \checkmark& 63.0 & 32.6 & 96.7 & 75.2 & 70.2 & 42.6 &  90.2 &56.3 & 90.0 & 75.0\\
% Mistral-7b & + w rationale & \checkmark& 39.0 & 30.1 & 90.0 & 79.3 & 54.4 & 46.5 & 75.7 & 61.8 & 78.0 & 76.0\\
% % Mistral-7b& + Test P \& S & \ding{55} &\\
% Mistral-7b&  + w rationale & \ding{55}& 50.0 & 26.9 & 97.5 & 80.1& 68.4 & 50.8 & 79.8 & 62.1 & 86.0 & 76.0\\
% \bottomrule
% \end{tabular}
% }
% \vspace{-2mm}
% \caption{Finetune performance (\%) (zero-shot) of Llama-2-7b-chat, Llama-2-13b-chat and Mistral-7b-instruction on the original and mimicked MMLU examples. Following setting in Table~\ref{tab: data leakge affect}.}
% \label{tab: data leakge affect mmlu}
% \vspace{-2mm}
% \end{table*}
\begin{table*}[htb]
 \vspace{-2mm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc|cc|cc|cc|cc}
\toprule
\textbf{Model} &\textbf{Training} & \textbf{LoRA Only}& \textbf{Algebra$_o$} &\textbf{Algebra$_m$}& \textbf{Law$_o$} &\textbf{Law$_m$}& \textbf{Econ$_o$} 
&\textbf{Econ$_m$} & \textbf{Medicine$_o$} &\textbf{Medicine$_m$}& \textbf{Security$_o$} &\textbf{Security$_m$}\\
 
\midrule
Llama2-7b & None & - &14.0 & 17.2 & 57.8 & 70.0 & 28.1 & 32.7 & 41.9 & 49.8 & 58.0 & 60.0 \\
% Llama-7b & + leakage & \checkmark & 52.0(\textcolor{red}{+38.0}) & 31.2(\textcolor{red}{+14.0}) & 95.9(\textcolor{red}{+38.1}) & 70.8(\textcolor{green}{+0.8}) & 65.8(\textcolor{red}{+37.7}) & 34.6(\textcolor{green}{+1.9}) & 79.8(\textcolor{red}{+37.9}) & 50.4(\textcolor{green}{+0.6}) & 86.0(\textcolor{red}{+28.0}) & 66.0(\textcolor{red}{+6.0})\\
% Llama-7b & + w rationale & \checkmark & 33.0(\textcolor{red}{+19.0}) & 30.1(\textcolor{red}{+12.9}) & 74.4(\textcolor{red}{+16.6}) & 72.7(\textcolor{green}{+2.7}) & 38.6(\textcolor{red}{+10.5}) & 31.7(\textcolor{green}{-1.0}) & 53.8(\textcolor{red}{+11.9}) & 50.8(\textcolor{green}{+1.0}) & 67.0(\textcolor{red}{+9.0}) & 60.0(\textcolor{green}{0.0})\\
% Llama-7b & + leakage & \ding{55} & 49.0(\textcolor{red}{+35.0}) & 23.7(\textcolor{red}{+6.5}) & 93.4(\textcolor{red}{+35.6}) & 70.9(\textcolor{green}{+0.9}) & 65.8(\textcolor{red}{+37.7}) & 33.6(\textcolor{green}{+0.9}) & 79.2(\textcolor{red}{+37.3}) & 51.1(\textcolor{green}{+1.3}) & 84.0(\textcolor{red}{+26.0}) & 60.0(\textcolor{green}{0.0})\\
% Llama-7b & + w rationale & \ding{55} & 42.0(\textcolor{red}{+28.0}) & 31.2(\textcolor{red}{+14.0}) & 81.8(\textcolor{red}{+24.0}) & 73.5(\textcolor{green}{+3.5}) & 46.5(\textcolor{red}{+18.4}) & 36.6(\textcolor{green}{+3.9}) & 62.4(\textcolor{red}{+20.5}) & 55.0(\textcolor{red}{+5.2}) & 76.0(\textcolor{red}{+18.0}) & 63.0(\textcolor{green}{+3.0})\\
% \midrule
% Llama-7b & + leakage & \checkmark & 52.0 (1) & 31.2 (2) & 95.9 (1) & 70.8 (4) & 65.8 (1) & 34.6 (4) & 79.8 (1) & 50.4 (4) & 86.0 (2) & 66.0 (3) \\
% Llama-7b & + w rationale & \checkmark & 33.0 (2) & 30.1 (2) & 74.4 (2) & 72.7 (4) & 38.6 (2) & 31.7 (5) & 53.8 (2) & 50.8 (4) & 67.0 (3) & 60.0 (4) \\
% Llama-7b & + leakage & \ding{55} & 49.0 (1) & 23.7 (3) & 93.4 (1) & 70.9 (4) & 65.8 (1) & 33.6 (4) & 79.2 (1) & 51.1 (4) & 84.0 (2) & 60.0 (4) \\
% Llama-7b & + w rationale & \ding{55} & 42.0 (2) & 31.2 (2) & 81.8 (2) & 73.5 (4) & 46.5 (2) & 36.6 (4) & 62.4 (2) & 55.0 (3) & 76.0 (2) & 63.0 (4) \\
Llama2-7b & + leakage & \checkmark & \cellcolor{lightred} 52.0 & \cellcolor{verylightred} 31.2 & \cellcolor{lightred} 95.9 & \cellcolor{lightblue} 70.8 & \cellcolor{lightred} 65.8 & \cellcolor{lightblue} 34.6 & \cellcolor{lightred} 79.8 & \cellcolor{lightblue} 50.4 & \cellcolor{verylightred} 86.0 & \cellcolor{extremelylightred} 66.0 \\
Llama2-7b & + w rationale & \checkmark & \cellcolor{verylightred} 33.0 & \cellcolor{verylightred} 30.1 & \cellcolor{verylightred} 74.4 & \cellcolor{lightblue} 72.7 & \cellcolor{verylightred} 38.6 & \cellcolor{medblue} 31.7 & \cellcolor{verylightred} 53.8 & \cellcolor{lightblue} 50.8 & \cellcolor{extremelylightred} 67.0 & \cellcolor{lightblue} 60.0 \\
Llama2-7b & + leakage & \ding{55} & \cellcolor{lightred} 49.0 & \cellcolor{extremelylightred} 23.7 & \cellcolor{lightred} 93.4 & \cellcolor{lightblue} 70.9 & \cellcolor{lightred} 65.8 & \cellcolor{lightblue} 33.6 & \cellcolor{lightred} 79.2 & \cellcolor{lightblue} 51.1 & \cellcolor{verylightred} 84.0 & \cellcolor{lightblue} 60.0 \\
Llama2-7b & + w rationale & \ding{55} & \cellcolor{verylightred} 42.0 & \cellcolor{verylightred} 31.2 & \cellcolor{verylightred} 81.8 & \cellcolor{lightblue} 73.5 & \cellcolor{verylightred} 46.5 & \cellcolor{lightblue} 36.6 & \cellcolor{verylightred} 62.4 & \cellcolor{extremelylightred} 55.0 & \cellcolor{verylightred} 76.0 & \cellcolor{lightblue} 63.0 \\
\midrule
Llama2-13b & None & - &31.0 & 29.0 & 70.0 & 77.8 & 30.0 & 36.7 & 43.6 & 50.1 & 65.0 & 72.0 \\
% Llama-13b & +leakage & \checkmark & 51.0(\textcolor{red}{+20.0}) & 30.1(\textcolor{green}{+1.1}) & 96.7(\textcolor{red}{+26.7}) & 79.5(\textcolor{green}{+1.7}) & 67.5(\textcolor{red}{+37.5}) & 42.5(\textcolor{red}{+5.8}) & 83.2(\textcolor{red}{+39.6}) & 54.9(\textcolor{green}{+4.8}) & 92.0(\textcolor{red}{+27.0}) & 76.0(\textcolor{green}{+4.0})\\
% Llama-13b & + w rationale & \checkmark & 34.0(\textcolor{green}{+3.0}) & 32.6(\textcolor{green}{+3.6}) & 86.0(\textcolor{red}{+16.0}) & 80.5(\textcolor{green}{+2.7}) & 39.5(\textcolor{red}{+9.5}) & 40.2(\textcolor{green}{+3.5}) & 58.4(\textcolor{red}{+14.8}) & 55.5(\textcolor{red}{+5.4}) & 75.0(\textcolor{red}{+10.0}) & 74.0(\textcolor{green}{+2.0})\\
% Llama-13b & +leakage & \ding{55} & 48.0(\textcolor{red}{+17.0}) & 23.7(\textcolor{green}{-5.3}) & 92.6(\textcolor{red}{+22.6}) & 70.9(\textcolor{green}{-6.9}) & 60.5(\textcolor{red}{+30.5}) & 36.6(\textcolor{green}{-0.1}) & 82.1(\textcolor{red}{+38.5}) & 50.4(\textcolor{green}{+0.3}) & 83.0(\textcolor{red}{+18.0}) & 71.0(\textcolor{green}{-1.0})\\
% Llama-13b & + w rationale & \ding{55} & 38.0(\textcolor{red}{+7.0}) & 35.4(\textcolor{red}{+6.4}) & 86.7(\textcolor{red}{+16.7}) & 80.1(\textcolor{green}{+2.3}) & 50.0(\textcolor{red}{+20.0}) & 40.5(\textcolor{green}{+3.8}) & 65.3(\textcolor{red}{+21.7}) & 55.6(\textcolor{red}{+5.5}) & 79.0(\textcolor{red}{+14.0}) & 74.0(\textcolor{green}{+2.0})\\
% \midrule
% Llama-13b & +leakage & \checkmark & 51.0(2) & 30.1(4) & 96.7(1) & 79.5(4) & 67.5(1) & 42.5(3) & 83.2(1) & 54.9(4) & 92.0(1) & 76.0(4)\\
% Llama-13b & + w rationale & \checkmark & 34.0(4) & 32.6(4) & 86.0(2) & 80.5(4) & 39.5(3) & 40.2(4) & 58.4(2) & 55.5(3) & 75.0(2) & 74.0(4)\\
% Llama-13b & +leakage & \ding{55} & 48.0(2) & 23.7(5) & 92.6(2) & 70.9(5) & 60.5(1) & 36.6(5) & 82.1(1) & 50.4(4) & 83.0(2) & 71.0(5)\\
% Llama-13b & + w rationale & \ding{55} & 38.0(3) & 35.4(3) & 86.7(2) & 80.1(4) & 50.0(2) & 40.5(4) & 65.3(2) & 55.6(3) & 79.0(2) & 74.0(4)\\
Llama2-13b & +leakage & \checkmark & \cellcolor{verylightred} 51.0 & \cellcolor{lightblue} 30.1 & \cellcolor{lightred} 96.7 & \cellcolor{lightblue} 79.5 & \cellcolor{lightred} 67.5 & \cellcolor{extremelylightred} 42.5 & \cellcolor{lightred} 83.2 & \cellcolor{lightblue} 54.9 & \cellcolor{lightred} 92.0 & \cellcolor{lightblue} 76.0\\
Llama2-13b & + w rationale & \checkmark & \cellcolor{lightblue} 34.0 & \cellcolor{lightblue} 32.6 & \cellcolor{verylightred} 86.0 & \cellcolor{lightblue} 80.5 & \cellcolor{extremelylightred} 39.5 & \cellcolor{lightblue} 40.2 & \cellcolor{verylightred} 58.4 & \cellcolor{extremelylightred} 55.5 & \cellcolor{verylightred} 75.0 & \cellcolor{lightblue} 74.0\\
Llama2-13b & +leakage & \ding{55} & \cellcolor{verylightred} 48.0 & \cellcolor{medblue} 23.7 & \cellcolor{verylightred} 92.6 & \cellcolor{medblue} 70.9 & \cellcolor{lightred} 60.5 & \cellcolor{medblue} 36.6 & \cellcolor{lightred} 82.1 & \cellcolor{lightblue} 50.4 & \cellcolor{verylightred} 83.0 & \cellcolor{medblue} 71.0\\
Llama2-13b & + w rationale & \ding{55} & \cellcolor{extremelylightred} 38.0 & \cellcolor{extremelylightred} 35.4 & \cellcolor{verylightred} 86.7 & \cellcolor{lightblue} 80.1 & \cellcolor{verylightred} 50.0 & \cellcolor{lightblue} 40.5 & \cellcolor{verylightred} 65.3 & \cellcolor{extremelylightred} 55.6 & \cellcolor{verylightred} 79.0 & \cellcolor{lightblue} 74.0\\

\midrule
Llama3-8b & None & - &34.0 & 36.5 & 76.9 & 82.0 & 50.9 & 59.4 & 65.9 & 70.3 & 74.0 & 81.0 \\
% Llama-8b & +leakage & \checkmark & 49.0 (\textcolor{red}{+15.0}) & 29.0 (\textcolor{green}{-7.5}) & 92.6 (\textcolor{red}{+15.7}) & 83.7 (\textcolor{green}{+1.7}) & 72.8 (\textcolor{red}{+21.9}) & 61.3 (\textcolor{green}{+1.9}) & 87.2 (\textcolor{red}{+21.3}) & 75.0 (\textcolor{green}{+4.7}) & 89.0 (\textcolor{red}{+15.0}) & 80.0 (\textcolor{green}{-1.0}) \\
% Llama-8b & + w rationale & \checkmark & 48.0 (\textcolor{red}{+14.0}) & 38.7 (\textcolor{green}{+2.2}) & 88.4 (\textcolor{red}{+11.5}) & 83.7 (\textcolor{green}{+1.7}) & 65.8 (\textcolor{red}{+14.9}) & 63.4 (\textcolor{green}{+4.0}) & 74.6 (\textcolor{red}{+8.7}) & 71.8 (\textcolor{green}{+1.5}) & 88.0 (\textcolor{red}{+14.0}) & 84.0 (\textcolor{green}{+3.0}) \\
% Llama-8b & + w rationale & \ding{55} & 54.0 (\textcolor{red}{+20.0}) & 39.7 (\textcolor{green}{+3.2}) & 90.1 (\textcolor{red}{+13.2}) & 87.2 (\textcolor{red}{+5.2}) & 74.6 (\textcolor{red}{+23.7}) & 61.3 (\textcolor{green}{+1.9}) & 76.3 (\textcolor{red}{+10.4}) & 75.6 (\textcolor{red}{+5.3}) & 80.0 (\textcolor{green}{+6.0}) & 83.0 (\textcolor{green}{+2.0}) \\
% \midrule
% Llama-8b   & None           & -        & 34.0 & 36.5 & 76.9 & 82.0 & 50.9 & 59.4 & 65.9 & 70.3 & 74.0 & 81.0  \\
% Llama-8b   & +leakage       & \checkmark & 49.0 (2) & 29.0 (5) & 92.6 (2) & 83.7 (4) & 72.8 (2) & 61.3 (4) & 87.2 (2) & 75.0 (4) & 89.0 (2) & 80.0 (5) \\
% Llama-8b   & + w rationale  & \checkmark & 48.0 (2) & 38.7 (4) & 88.4 (2) & 83.7 (4) & 65.8 (2) & 63.4 (4) & 74.6 (3) & 71.8 (4) & 88.0 (2) & 84.0 (4) \\
% Llama-8b   & + w rationale  & \ding{55}  & 54.0 (2) & 39.7 (4) & 90.1 (2) & 87.2 (3) & 74.6 (2) & 61.3 (4) & 76.3 (2) & 75.6 (3) & 80.0 (3) & 83.0 (4) \\
Llama3-8b   & +leakage       & \checkmark & \cellcolor{verylightred}49.0 & \cellcolor{medblue}29.0 & \cellcolor{verylightred}92.6 & \cellcolor{lightblue}83.7 & \cellcolor{verylightred}72.8 & \cellcolor{lightblue}61.3 & \cellcolor{verylightred}87.2 & \cellcolor{lightblue}75.0 & \cellcolor{verylightred}89.0 & \cellcolor{medblue}80.0 \\
Llama3-8b   & + w rationale  & \checkmark & \cellcolor{verylightred}48.0 & \cellcolor{lightblue}38.7 & \cellcolor{verylightred}88.4 & \cellcolor{lightblue}83.7 & \cellcolor{verylightred}65.8 & \cellcolor{lightblue}63.4 & \cellcolor{extremelylightred}74.6 & \cellcolor{lightblue}71.8 & \cellcolor{verylightred}88.0 & \cellcolor{lightblue}84.0 \\
Llama3-8b   & + w rationale  & \ding{55}  & \cellcolor{verylightred}54.0 & \cellcolor{lightblue}39.7 & \cellcolor{verylightred}90.1 & \cellcolor{extremelylightred}87.2 & \cellcolor{verylightred}74.6 & \cellcolor{lightblue}61.3 & \cellcolor{verylightred}76.3 & \cellcolor{extremelylightred}75.6 & \cellcolor{extremelylightred}80.0 & \cellcolor{lightblue}83.0 \\
\midrule
Mistral-7b & None & - & 34.0 & 26.8 & 70.2 & 77.1 & 36.9 & 45.7 & 59.5 & 59.3 & 70.0 & 74.0 \\
% Mistral-7b & + leakage & \checkmark & 63.0(\textcolor{red}{+29.0}) & 32.6(\textcolor{red}{+5.8}) & 96.7(\textcolor{red}{+26.5}) & 75.2(\textcolor{green}{-1.9}) & 70.2(\textcolor{red}{+33.3}) & 42.6(\textcolor{green}{-3.1}) & 90.2(\textcolor{red}{+30.7}) & 56.3(\textcolor{green}{-3.0}) & 90.0(\textcolor{red}{+20.0}) & 75.0(\textcolor{green}{+1.0}) \\
% Mistral-7b & + w rationale & \checkmark & 39.0(\textcolor{red}{+5.0}) & 30.1(\textcolor{green}{+3.3}) & 90.0(\textcolor{red}{+19.8}) & 79.3(\textcolor{green}{+2.2}) & 54.4(\textcolor{red}{+17.5}) & 46.5(\textcolor{green}{+0.8}) & 75.7(\textcolor{red}{+16.2}) & 61.8(\textcolor{green}{+2.5}) & 78.0(\textcolor{red}{+8.0}) & 76.0(\textcolor{green}{+2.0}) \\
% Mistral-7b & + w rationale & \ding{55} & 50.0(\textcolor{red}{+16.0}) & 26.9(\textcolor{green}{+0.1}) & 97.5(\textcolor{red}{+27.3}) & 80.1(\textcolor{green}{+3.0}) & 68.4(\textcolor{red}{+31.5}) & 50.8(\textcolor{red}{+5.1}) & 79.8(\textcolor{red}{+20.3}) & 62.1(\textcolor{green}{+2.8}) & 86.0(\textcolor{red}{+16.0}) & 76.0(\textcolor{green}{+2.0}) \\
% \midrule
% Mistral-7b & + leakage & \checkmark & 63.0 (2) & 32.6 (3) & 96.7 (2) & 75.2 (5) & 70.2 (1) & 42.6 (5) & 90.2 (1) & 56.3 (5) & 90.0 (2) & 75.0 (4) \\
% Mistral-7b & + w rationale & \checkmark & 39.0 (3) & 30.1 (4) & 90.0 (2) & 79.3 (4) & 54.4 (2) & 46.5 (4) & 75.7 (2) & 61.8 (4) & 78.0 (3) & 76.0 (4) \\
% Mistral-7b & + w rationale & \ding{55} & 50.0 (2) & 26.9 (4) & 97.5 (2) & 80.1 (4) & 68.4 (1) & 50.8 (3) & 79.8 (2) & 62.1 (4) & 86.0 (2) & 76.0 (4) \\
Mistral-7b & + leakage & \checkmark & \cellcolor{verylightred} 63.0 & \cellcolor{extremelylightred} 32.6 & \cellcolor{verylightred} 96.7 & \cellcolor{medblue} 75.2 & \cellcolor{lightred} 70.2 & \cellcolor{medblue} 42.6 & \cellcolor{lightred} 90.2 & \cellcolor{medblue} 56.3 & \cellcolor{verylightred} 90.0 & \cellcolor{lightblue} 75.0 \\
Mistral-7b & + w rationale & \checkmark & \cellcolor{extremelylightred} 39.0 & \cellcolor{lightblue} 30.1 & \cellcolor{verylightred} 90.0 & \cellcolor{lightblue} 79.3 & \cellcolor{verylightred} 54.4 & \cellcolor{lightblue} 46.5 & \cellcolor{verylightred} 75.7 & \cellcolor{lightblue} 61.8 & \cellcolor{extremelylightred} 78.0 & \cellcolor{lightblue} 76.0 \\
Mistral-7b & + w rationale & \ding{55} & \cellcolor{verylightred} 50.0 & \cellcolor{lightblue} 26.9 & \cellcolor{verylightred} 97.5 & \cellcolor{lightblue} 80.1 & \cellcolor{lightred} 68.4 & \cellcolor{extremelylightred} 50.8 & \cellcolor{verylightred} 79.8 & \cellcolor{lightblue} 62.1 & \cellcolor{verylightred} 86.0 & \cellcolor{lightblue} 76.0 \\

\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Finetune performance (\%) of Llama-2-7b-chat, Llama-2-13b-chat, Llama-3-8b-Instruction and Mistral-7b-instruction on the mimicked MMLU examples. Following the setting in Table~\ref{tab: data leakge affect}.}
\label{tab: data leakge affect mmlu}
\vspace{-6mm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Extending Strategy: Stability \& Dealing with Data Leakage }\label{sec: extending}
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2mm}
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcc|c|c}
\toprule 
\textbf{Model} &  \textbf{Training} &\textbf{LoRA only} &\textbf{Algebra} & \textbf{Algos} \\
\midrule

Llama2-7b & None & -& \textbf{4.2} $\pm{0.6}$ & \textbf{10.2} $\pm{0.5}$ \\
Llama2-7b & + leakage & \checkmark & 1.6 $\pm{0.6}$  & 2.2 $\pm{0.6}$\\
Llama2-7b & + w rationale & \checkmark& 1.2 $\pm{0.0}$ & 5.3 $\pm{0.5}$\\
Llama2-7b & + leakage & \ding{55} & 1.8 $\pm{0.6}$ &1.1 $\pm{0.0}$ \\
Llama2-7b & + w rationale & \ding{55} & 2.1 $\pm{0.5}$ & 8.9 $\pm{0.8}$\\
\midrule
Llama2-13b& None &-  & \textbf{8.5}  $\pm{0.4}$& \textbf{11.9} $\pm{0.8}$ \\
Llama2-13b& + leakage & \checkmark& 6.6 $\pm{0.5}$ & 5.1 $\pm{0.1}$\\
Llama2-13b&  + w rationale& \checkmark & 6.4 $\pm{0.9}$& 11.2 $\pm{0.8}$\\
Llama2-13b& + leakage & \ding{55} & 1.5 $\pm{0.4}$& 0.5 $\pm{0.4}$\\
Llama2-13b&  + w rationale& \ding{55} & 5.7 $\pm{0.5}$& 7.7 $\pm{1.2}$\\
\midrule
Llama3-8b& None &-  & \textbf{34.6}  $\pm{1.6}$& \textbf{46.7} $\pm{2.1}$ \\
Llama3-8b& + leakage & \checkmark& 12.1 $\pm{0.5}$ & 21.3 $\pm{2.2}$\\
Llama3-8b&  + w rationale& \checkmark & 17.8 $\pm{1.3}$& 17.5 $\pm{1.8}$\\
Llama3-8b&  + w rationale& \ding{55} & 15.3 $\pm{1.6}$& 18.7 $\pm{1.2}$\\
% LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
\midrule
Mistral-7b & None & -& \textbf{21.8} $\pm{1.7}$  & \textbf{36.8} $\pm{0.0}$\\
Mistral-7b & + leakage & \checkmark & 0.9 $\pm{0.5}$ &  5.3 $\pm{0.5}$\\
Mistral-7b &  + w rationale& \checkmark  & 4.4 $\pm{0.6}$ &  9.1 $\pm{0.5}$\\
Mistral-7b &  + w rationale& \ding{55}  & 2.3 $\pm{0.2}$& 4.4 $\pm{0.8}$\\
\bottomrule
\end{tabular} }
\vspace{-2mm}
\captionof{table}{Average percentage (\%)  of full-mark of the fine-tuned model on the extended dataset over the four iterations.}
\label{tab: data leakage extend}
\vspace{-5mm}
\end{wrapfigure}
As shown in Section~\ref{Sec: how data leakage affect}, the mimicking strategy does not work well on two datasets: Algos and Algebra. The data leakage issue still leads to the severe overestimation of model, which we will further explore using the extending strategy in this section. Following the experiment settings of the mimicking strategy, we leverage the same baseline models with leakage simulations, as well as four iterations of dataset updates for stability verification (updating process defined in Section~\ref{Extend setting} and Section~\ref{sec: Updated Dataset Analysis} and statistical details can be found in Table~\ref{table: extend data all}). As shown in Table~\ref{tab: data leakage extend}, the standard deviation among four runs is quite low, demonstrating the stability of our extending strategy. This is not surprising as extending strategy can be regarded as an extension of the mimicking strategy with varying cognitive levels for controllable difficulty (Section~\ref{sec diff}). 

To investigate the effectiveness, we employ baseline models in the mimicking strategy that are fine-tuned on test samples from the original datasets. Table~\ref{tab: data leakage extend} shows that all performances of leakage simulations greatly decrease compared with original models due to the overfitting issue. Moreover, the decline of \textit{leakage} is more than that of \textit{w rationale} because it is alleviated through the improved generalization ability via learning with rationales. However, note that even with rationales, the model still exhibits signs of overfitting, which may improve its performance on the original test set. 

% \subsection{Can we control the question difficulty using the extend setting?} \label{sec diff}
\subsection{Is that possible to control the sample difficulty using the Extending Strategy?} \label{sec diff}
\begin{figure}[htb]
\centering
\includegraphics[scale=0.20]{figures/extend_result_flat.pdf}
\vspace{-2mm}
    \caption{Rull-mark rate (\%) of the mode GPT-4, ChatGPT, Claude and Gemini on the extended Sports datasets (a) and Phys (b) on different cognitive levels.}
    \label{fig: extend result}  
\vspace{-2mm}
\end{figure}

Except for overestimation leading by data leakage in Section~\ref{sec: extending}, there is another issue on the task Sports and Phys (Table~\ref{tab: data leakge affect} and Table~\ref{tab: data leakge affect mmlu})  --- the absolute scores are quite high so that models' performance cannot be distinguished well (i.e., 3.82\% and 4.30\% difference on average for models GPT-4, ChatGPT, Gemini, and Claude). 
% In this section, we explore how to control the difficulty of extended datasets from two aspects: \textbf{1)} adjusting the cognitive levels, more abstract levels are expected to produce more difficult samples; and \textbf{2)} entity popularity, questions about long-tail entities are much more difficult to answer for LLMs~\cite{mallennot}. Specifically, we use the extracted sports star name and the summarized common physical law as the seed and update the dataset using extending strategy (Section~\ref{sec Updated Dataset Analysis}). We use models GPT-4, ChatGPT, Gemini, and Claude as the baseline for their indistinguishable performance.
In this section, we demonstrate the feasibility of controlling the difficulty of the extended data sample from two perspectives: 1) Work~\cite{krathwohl2002revision} suggests that cognitive demand increases with higher cognitive processes. Accordingly, by adjusting to more abstract cognitive levels, we expect to produce more challenging samples. 2) Work~\cite{mallennot} indicates that as the popularity of the subject entity increases, the difficulty of the question decreases. 

To validate the efficacy of our approach in controlling difficulty, we use the extracted sports star name and the summarized common physical law as the seed to update the dataset using the extending strategy (Section~\ref{sec: Updated Dataset Analysis}). We use models GPT-4, ChatGPT, Gemini, and Claude as the baseline for their indistinguishable performance.
% \yixin{As shown in Figure~\ref{fig: extend result}, we can see }
As shown in Figure~\ref{fig: extend result}, \textbf{1)} on the extended Sports and Phys dataset, the four models' performance show larger variance (23.76\%, 14.04\% respectively), compared with it on original datasets; \textbf{2)} overall, samples test ``Apply'' and ``Evaluation'' cognitive levels are found to be more challenging. This finding indicates that manipulating the cognitive level in the extending strategy is an effective way of controlling the difficulty of the questions. It also highlights the importance of focusing on models' capabilities across different cognitive levels. Some models exhibit significant disparities in performance across various cognitive levels, while GPT-4  shows stronger performance. 
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2mm}
\includegraphics[scale=0.28]{figures/pop.pdf} 
\caption{Rull-mark rate (\%) of GPT-4, ChatGPT, Claude and Gemini on the extended ``sport understanding'' datasets on different popularity levels. We depict the number of questions on different popularity levels.}
\label{fig: pop result} 
\end{wrapfigure}
% \begin{figure}[htb]
% \centering
% \begin{minipage}[t]{0.48\textwidth}
% \includegraphics[scale=0.28]{figures/pop.pdf}
%     \caption{Rull-mark rate (\%) of GPT-4, ChatGPT, Claude and Gemini on the extended ``sport understanding'' datasets on different popularity levels. We depict the number of questions on different popularity levels.}
%     \label{fig: pop result} 
% \end{minipage}
% \begin{minipage}[t]{0.48\textwidth}
% \end{minipage}
% \end{figure} 
In addition to assessing how cognitive levels influence performance, we explored how the popularity of the seeds used in 
% question generation 
dataset update affects model performance. Following previous work~\cite{mallennot}, where using Wikipedia page views as a measure of popularity, we gather the total page views for each seed throughout the year 2023 and use it as the popularity. As shown in Figure~\ref{fig: pop result}, despite an uneven distribution of seed popularity in the extended dataset, a clear trend emerged: there was a noticeable increase in model performance when using more popular seeds to get the question. 
This observation suggests that the popularity of the seed input can also be strategically manipulated to control the difficulty of the generated questions. 
% \begin{figure}[ht]
% \begin{minipage}{0.50\textwidth}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|c|c|c}
% \toprule
% \textbf{Dataset} & \textbf{\#Total} & \textbf{\#Clean}& 
% \textbf{\#Input} 
% \textbf{Dirty}
%  &  \textbf{\#Input-label Dirty} \\  
% \midrule
% Algebra & 80& 80& 0 &0\\
% Algos & 320 & 320&0 &0 \\
% Phys & 80 & 79& 1 & 0\\
% Sports & 824 & 824& 0 &0\\
% \bottomrule
% \end{tabular}}
% % \begin{tabular}{l|c|c|c|c}
% % \toprule
% %  & \textbf{Algebra} & \textbf{Algos} & \textbf{Phys} & \textbf{Sports} \\
% % \midrule
% % \textbf{\#Total} & 80 & 320 & 80 & 824 \\
% % \textbf{\#Clean} & 80 & 320 & 79 & 824 \\
% % \textbf{\#Input Dirty} & 0 & 0 & 1 & 0 \\
% % \textbf{\#Input-label Dirty} & 0 & 0 & 0 & 0 \\
% % \bottomrule
% % \end{tabular}}

% \captionof{table}{The contamination report on the extended data samples. We compare the generated sample with the web source, the benchmark source, and IFT dataset.}
% \label{tab: containmation}
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\textwidth}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcc|c}
% \toprule 
% \textbf{Model} &  \textbf{Training} &\textbf{LoRa only} &\textbf{Algebra} \\
% \midrule

% Llama-7b & None & -& \textbf{26.3}  $\pm{1.6}$ \\

% Llama-7b & + w rationale & \checkmark & 8.9 $\pm {0.5}$ \\
% Llama-7b & + w rationale & \ding{55} & 22.1 $\pm {0.5}$ \\
% \midrule
% Llama-13b& None &-  & \textbf{33.9}  $\pm {1.9}$  \\
% Llama-13b&  + w rationale& \checkmark & 26.0 $\pm {1.0}$  \\
% Llama-13b&  + w rationale& \ding{55} & 9.7  $\pm {1.6}$ \\
% \midrule
% Llama3-8b& None &- & \textbf{59.0} $\pm {1.5}$\\
% Llama3-8b&  + w rationale& \checkmark & 39.6 $\pm {0.4}$  \\
% Llama3-8b&  + w rationale& \ding{55} & 41.1  $\pm {1.0}$ \\
% % LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
% \midrule
% Mistral-7b & None & -& \textbf{45.5} $\pm {0.4}$ \\
% Mistral-7b &  + w rationale& \checkmark   & 17.9 $\pm {0.4}$\\
% Mistral-7b &  + w rationale& \ding{55}  & 6.8 $\pm {2.2}$\\
% \bottomrule
% \end{tabular} 
% }
% \captionof{table}{Average percentage (\%)  of full-mark of the fine-tuned model on the extended dataset from Claude3 as examiner}
% \label{tab: data leakage extend claude3}
% \end{minipage}
% \end{figure}


 \subsection{Adaptable to Models Beyond the GPT Backbone}\label{sec: Adaptable to models beyond the GPT backbone}
Relying solely on ChatGPT or GPT-4 may introduce biases, such as self-preference, particularly when employing the 'LLM-as-an-Examiner' methodology~\cite{bai2023benchmarking}. Thus we expand the experimentation by using Claude-3-Opus~\citep{Claude-3} to generate new samples, demonstrating the framework's adaptability 
\begin{wrapfigure}{r}{0.35\textwidth}
\centering
\resizebox{0.35\textwidth}{!}{%
\begin{tabular}{lcc|c|c}
\toprule 
\textbf{Model} &  \textbf{Training} &\textbf{LoRA only} &\textbf{Algebra} \\
\midrule

Llama2-7b & None & -& \textbf{26.3}  $\pm{1.6}$ \\

Llama2-7b & + w rationale & \checkmark & 8.9 $\pm {0.5}$ \\
Llama2-7b & + w rationale & \ding{55} & 22.1 $\pm {0.5}$ \\
\midrule
Llama2-13b& None &-  & \textbf{33.9}  $\pm {1.9}$  \\
Llama2-13b&  + w rationale& \checkmark & 26.0 $\pm {1.0}$  \\
Llama2-13b&  + w rationale& \ding{55} & 9.7  $\pm {1.6}$ \\
\midrule
Llama3-8b& None &- & \textbf{59.0} $\pm {1.5}$\\
Llama3-8b&  + w rationale& \checkmark & 39.6 $\pm {0.4}$  \\
Llama3-8b&  + w rationale& \ding{55} & 41.1  $\pm {1.0}$ \\
% LLamA-13b with e + a & 96.6 & 95.4 & 48.5 & 4.4 & 23.1 & 18 & 98.6 & 96.2 & 83.9 & 73.4 & 46.8 & 36.6 \\
\midrule
Mistral-7b & None & -& \textbf{45.5} $\pm {0.4}$ \\
Mistral-7b &  + w rationale& \checkmark   & 17.9 $\pm {0.4}$\\
Mistral-7b &  + w rationale& \ding{55}  & 6.8 $\pm {2.2}$\\
\bottomrule
\end{tabular} }
\captionof{table}{Average performance (\%) (full-mark rate) of the fine-tuned models on the extended datasets generated by Claude-3-Opus over the two iterations.}
\label{tab: data leakage extend claude3}
\end{wrapfigure}
and reliability. Using Claude-3-Opus we extend the algebra task, where the mimicking strategy is less effective, following the setting in Section~\ref{Sec: how data leakage affect}. Due to time and cost considerations, we only conduct the generation process two times, the static result is shown in Table~\ref{table: extend data all}.  We deploy models that are fine-tuned on test samples from the original datasets with rationales (\textit{w rationale}), which demonstrated superior performance compared to \textit{leakage} simulations to investigate the effectiveness. Shown in Table~\ref{tab: data leakage extend claude3}, the performance of the leakage simulations significantly declined compared to the original models, indicating the adaptability of our framework of using other models as backbone.

\vspace{-2mm}
\subsection{Does the extended data sample have data leakage problem?}\label{comtainmation report}
\vspace{-2mm}
If the generated samples are from some of the pre-trained datasets, it will lead to potential data leakage problems. In this section, we measure the potential data leakage in these extended 
% questions, 
samples\footnote{Considering the time and cost, we only use the first iteration, which statistics is shown in Table~\ref{table: mimic data})}.
Following previous work~\cite{li2023open, dodge2021documenting}, we calculate the similarity between newly generated data and data from public sources. We involve public data from three sources: web data, public benchmarks, and Instruction Fine-Tuning (IFT) data. For web data, we  extracted relevant queries 
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2mm}
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Dataset} & \textbf{\#Total} & \textbf{\#Clean}& 
\textbf{\#Input} 
\textbf{Dirty}
 &  \textbf{\#Input-label Dirty} \\  
\midrule
Algebra & 154 & 154& 0 &0\\
Algos & 320 & 320&0 &0 \\
Phys & 80 & 79& 1 & 0\\
Sports & 824 & 824& 0 &0\\
\bottomrule
\end{tabular}}
\captionof{table}{The contamination report on the extended data samples. We compare the generated sample with the web, benchmark, and IFT dataset source.}
\label{tab: containmation}
\vspace{-3mm}
\end{wrapfigure}
and context through Bing searches API, for public benchmarks we select several popular benchmarks: MMLU, HellaSwag~\cite{zellers2019hellaswag}, BIG-bench, ARC~\cite{clark2018think}, CommonsenseQA~\cite{commonsenseqa}, Winogrande~\cite{sakaguchi2021winogrande}, and for IFT dataset we select LaMini-Instruction~\citep{lamini-lm}, WizardLM-evol-instruct-V2~\cite{xu2023wizardlm}, and P3~\cite{sanh2021multitask}.
Following the methodology in \cite{li2023open}, we utilize Meteor \cite{meteor} as our similarity metric, and use the same parameter setting in \cite{li2023open}. We categorized the generated samples following~\cite{dodge2021documenting}:
\textbf{Clean:} No contamination present. \textbf{Input Dirty:} Only the question appears in the public data.\textbf{Input-and-Label Dirty:} Both question and answer are found in the public data. As evidenced in Table~\ref{tab: containmation}, extending strategy won't have data leakage issue.


% \begin{table}[htbp]
% \centering
% \caption{Aligning around the $\pm$ symbol}
% \begin{tabular}{lccR{0.2cm}@{$\pm$}L{1.2cm}R{1.2cm}@{$\pm$}L{1.2cm}}
% \toprule
% \textbf{Model} & \textbf{Training} & \textbf{LoRa only} & \multicolumn{2}{c}{\textbf{Algebra}} & \multicolumn{2}{c}{\textbf{Algos}} \\
% \midrule
% Llama-7b    & None         & -          & 4.2 & 0.6 & 10.2 & 0.5 \\
% Llama-7b    & + leakage    & \checkmark & 1.6 & 0.6 &  2.2 & 0.6 \\
% Llama-7b    & + w rationale& \checkmark & 1.2 & 0.0 &  5.3 & 0.5 \\
% Llama-7b    & + leakage    & \ding{55}  & 1.8 & 0.6 &  1.1 & 0.0 \\
% Llama-7b    & + w rationale& \ding{55}  & 2.1 & 0.5 &  8.9 & 0.8 \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{wrapfigure}{r}{0.5\textwidth}
% \centering
% \caption{Aligning around the $\pm$ symbol}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcc|R{0.8cm}@{$\pm$}L{0.8cm}R{0.8cm}@{$\pm$}L{0.8cm}}
% \toprule
% \textbf{Model} & \textbf{Training} & \textbf{LoRa only} & \multicolumn{2}{c}{\textbf{Algebra}} & \multicolumn{2}{c}{\textbf{Algos}} \\
% \midrule
% Llama-7b    & None         & -          & 4.2 & 0.6 & 10.2 & 0.5 \\
% Llama-7b    & + leakage    & \checkmark & 1.6 & 0.6 &  2.2 & 0.6 \\
% Llama-7b    & + w rationale& \checkmark & 1.2 & 0.0 &  5.3 & 0.5 \\
% Llama-7b    & + leakage    & \ding{55}  & 1.8 & 0.6 &  1.1 & 0.0 \\
% Llama-7b    & + w rationale& \ding{55}  & 2.1 & 0.5 &  8.9 & 0.8 \\
% \bottomrule
% \end{tabular}}
% \end{wrapfigure}



==> chapters/intro.tex <==
\section{Introduction} \label{sec: Introduction}
Large Language Models (LLMs) have become essential tools in the field of Natural Language Processing, marking significant advancements as highlighted by a series of influential studies~\citep{brown2020language, weichain, mirowski2023co}. Trained on wide-ranging datasets, these models exhibit 
% remarkable emergent abilities, including 
 in-context learning, instruction following, and step-by-step reasoning capabilities~\citep{wei2022emergent, zhao2023survey}. As the pre-trained data and capabilities of LLMs expand, how to curate suitable datasets for evaluation is becoming more and more challenging. On one hand, as highlighted by~\citep{li2023open, 
zhou2023don, wei2023skywork, li2023task, jacovi2023stop}, data leakage or contamination, the phenomenon that examples from the evaluation set are also found in the training set~\citep{li2023open}, leads to overestimations of LLM performance. A straightforward solution, on the other hand, is to manually update the dataset at regular intervals to alleviate the overestimation, which is costly.

In this paper, we aim to automate dataset updates for evaluation reliability and timeliness. When facing data leakage issues, we can simply replace compromised data without costly human efforts. Compared with building from scratch, our proposal is based on existing benchmarks, offering a more practical solution with minimal human effort. However, this is non-trivial due to the following research questions. 

\begin{itemize}
    \item Can the updated datasets alleviate overestimation when data leakage happens?

    \item Is it stable if we dynamically update evaluation datasets?

   \item Can automatically update datasets better discern and differentiate model capabilities?
\end{itemize}


To this end, we propose two strategies based on cognitive theory, mimicking and extending a given dataset, toward reliable and timely evaluation. i) Our \textbf{mimicking} strategy is to leverage LLMs to generate similar ones for each existing sample (marked as seeds), so that we, to the maximum extent, preserve the stylistic and contextual essence of the original data. This is simple and efficient, while it is under exploration if the overestimation caused by data leakage can be mitigated. ii) Our \textbf{extending} strategy further expands the original data according to varying cognitive levels. Here, we borrow the concepts from Bloom's taxonomy, \textit{a hierarchical classification widely used for educational learning objectives into levels of complexity and specificity.} This not only makes our evaluation more systematic but also leads to a balanced difficulty of the dataset, which can better distinguish and analyze the capabilities of models --- neither too difficult nor too easy can fairly judge students' learning status.

For evaluation, we systematically investigate the above two strategies regarding effectiveness, stability, and their abilities to deal with overestimation when data leakage happens. We generate datasets based on two widely used benchmarks (i.e., MMLU~\citep{hendryckstest2021} and BIG-Bench~\citep{srivastava2023beyond}), and study seven open-source models and four closed-source models.
We find that: \textbf{1)} Both mimicking and extending strategies show a high level of stability (Section~\ref{sec: stable evaluation} \& ~\ref{sec: extending}). \textbf{2)} The mimicking strategy is effective in alleviating overestimation. In most cases, compared with the leaked original dataset, there is no significant performance improvement on our updated one (Section~\ref{Sec: how data leakage affect})
\textbf{3)} While, in the cases where the mimicking dataset also shows enhanced performance, our extending strategy can still effectively deal with the overestimation issue (Section~\ref{sec: extending}). \textbf{4)} We can manipulate Bloom's concept of a sample and the popularity of seeds to control the difficulty of the extended dataset. The experimental results also provide a fine-grained analysis of LLMs' cognitive levels. Some models demonstrate considerable variations in their performance across different cognitive levels, yet GPT-4 exhibits strong performance across all levels (Section~\ref{sec diff}). Our main contributions can be summarized:
\begin{itemize}
  
    \item To the best of our knowledge, we are the first to automate dataset updates to alleviate the issue of overestimation when data leakage happens. 

%     We propose two strategies to automate dataset updates to alleviate data leakage issue during62
% evaluation.

    \item We propose to control the difficulty of the sample using varying cognitive levels, toward fair and fine-grained analysis. 

    \item We have conducted extensive experiments, demonstrating the effectiveness and stability of our two strategies.

\end{itemize}
